Modal Logics with Composition on Finite Forests: Expressivity and Complexity (Extra Material)

We investigate the expressivity and computational complexity of two modal logics on finite forests equipped with operators to reason on submodels. The logic ML(|) extends the basic modal logic ML with the composition operator | from static ambient logic, whereas ML(*) contains the separating conjunction * from separation logic. Though both operators are second-order in nature, we show that ML(|) is as expressive as the graded modal logic GML (on finite trees) whereas ML(*) lies strictly between ML and GML. Moreover, we establish that the satisfiability problem for ML(*) is Tower-complete, whereas for ML(|) is (only) AExpPol-complete. As a by-product, we solve several open problems related to sister logics, such as static ambient logic, modal separation logic, and second-order modal logic on finite trees.

==> proofs/proof-MSOK.tex <==
The proof of \Cref{corr:MSOK-tower} is quite straightforward. First, we recall that
$\arelation|_{\aworld}^{\leq n} \egdef \{\pair{\aworld'}{\aworld''} \in \arelation \mid \aworld' \in \arelation^{i}(\aworld) \text{ for some } i \in \interval{0}{n-1} \}$,
as defined in Appendix~\ref{appendix-preliminary-proofs}.
We write $\ML(\separate,\chopop)$ for the logic that extends $\ML$ with both $\separate$ and $\chopop$.

Let $\aformula$ be a formula in $\ML(\separate,\chopop)$. W.l.o.g.\ we can assume that $\aformula$ does not contain atomic propositions from $\apropsetbis = \{\avarpropbis_1,\avarpropbis_2,\avarpropbis_3\}$.
Let $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ be a finite forest and $\aworld \in \worlds$.
Let $\amodel' = \triple{\worlds'}{\arelation'}{\avaluation'}$ be a finite forest such that $\arelation'$ is connected, so that $\amodel$ is a \emph{ finite tree} (i.e. a model of $\msokt$), and let $\aworld' \in \worlds'$.
Given $n \in \Nat$ and $i \in \interval{1}{3}$, we say that $\pair{\amodel'}{\aworld'}$ is a $(n,i)$-\emph{encoding}
of $\pair{\amodel}{\aworld}$ if and only if there is a tree isomorphism $\amap$ between the trees described by $\arelation|_{\aworld}^{\leq n}$ and $\arelation'[i]|_{\aworld'}^{\leq n}$ (where
   $\arelation'[i] \egdef \{\pair{\aworld_1}{\aworld_2} \in \arelation' \mid \aworld_2 \in \avaluation(\avarpropbis_i)\}$), $\amap(\aworld) = \aworld'$ and
for every $\avarprop \in \AP \setminus \apropsetbis$ and every
$\aworld' \in (\arelation|_{\aworld}^{\leq n})^*(\aworld)$,
$\aworld'
\in \avaluation(\avarprop) \iff \amap(\aworld') \in \avaluation'(\avarprop)$.
Notice that $(\arelation|_{\aworld}^{\leq n})^*(\aworld)$ corresponds to the set of worlds appearing in $\arelation|_{\aworld}^{\leq n}$.
Moreover, for every $n \geq 2$, if $\pair{\amodel'}{\aworld'}$ is a $(n,i)$-encoding
of $\pair{\amodel}{\aworld}$ then
$\pair{\amodel'}{\aworld'}$ is a $(n-1,i)$-encoding
of $\pair{\amodel}{\aworld}$.

\begin{lemma}\label{A:lemma:MSOK-induction}
  Let $\aformula$ in $\ML(\separate,\chopop)$. Let $\apropsetbis = \{\avarpropbis_1,\avarpropbis_2,\avarpropbis_3\}$ be three atomic propositions not appearing in $\aformula$.
  Let $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ be a finite forest and $\aworld \in \worlds$.
  Let $\amodel' = \triple{\worlds'}{\arelation'}{\avaluation'}$ and $\aworld' \in \worlds'$ such that $\pair{\amodel'}{\aworld'}$ is a $(n,i)$-encoding of $\pair{\amodel}{\aworld}$, for some $n \geq \md{\aformula}$.
  Then,
  \begin{nscenter}
      $\amodel,\aworld \models \aformula \iff \amodel',\aworld' \models \atranslation_i(\aformula)$.
  \end{nscenter}
\end{lemma}

\begin{proof}
The proof follows with an easy structural induction on $\aformula$.
Let us develop the most interesting (inductive) case, i.e.\ when $\aformula = \aformula_1 \chopop \aformula_2$.
Let $\amap$ be the tree isomorphism witnessing that $\pair{\amodel'}{\aworld'}$ is a $(\md{\aformula},i)$-encoding of $\pair{\amodel}{\aworld}$.
\begin{description}
\item[($\Rightarrow$):] Suppose $\amodel,\aworld \models \aformula_1 \chopop \aformula_2$. By definition, there are $\amodel_1 = \triple{\worlds}{\arelation_1}{\avaluation}$, $\amodel_2 = \triple{\worlds}{\arelation_2}{\avaluation}$ s.t. $\amodel = \amodel_1 +_{\aworld} \amodel_2$,
$\amodel_1, \aworld \models \aformula_1$ and $\amodel_2, \aworld \models \aformula_2$.
Let $j,k \in \interval{1}{3}$ so that $j < k$ and $j \neq i \neq k$.
Let us consider the model $\amodel'' = \triple{\worlds'}{\arelation'}{\avaluation''}$ obtained from $\amodel'$ by updating the valuation $\avaluation'(\avarpropbis_j)$ and $\avaluation'(\avarpropbis_k)$ as follows:
\begin{nscenter}
  $\avaluation''(\avarpropbis_j) = \{ \amap(\aworld'') \mid \exists \overline{\aworld} \text{ s.t.\ } \pair{\overline{\aworld}}{\aworld''} \in \arelation_1 \}$;
  \qquad\quad
  $\avaluation''(\avarpropbis_k) = \worlds \setminus \avaluation''(\avarpropbis_j)$.
\end{nscenter}
By definition it is easy to see that $\amodel'',\aworld' \models [\avarpropbis_i = \avarpropbis_j + \avarpropbis_k]^{\md{\aformula_1 \chopop \aformula_2}}$.
Similarly, we can easily show that $\pair{\amodel''}{\aworld'}$ is a $\pair{\md{\aformula_1 \chopop \aformula_2}}{j}$-encoding of $\pair{\amodel_1}{\aworld}$, as
well as a $\pair{\md{\aformula_1 \chopop \aformula_2}}{k}$-encoding of $\pair{\amodel_2}{\aworld}$.
Then, by inductive hypothesis $\amodel'',\aworld' \models \atranslation_j(\aformula_1) \land \atranslation_k(\aformula_2)$.
Moreover, by definition of $+_{\aworld}$ and since $\amodel_1 +_{\aworld} \amodel_2$, for every $l \in \{1,2\}$ and $\aworld_1 \in \worlds$ if $\pair{\aworld}{\aworld_1} \in \arelation_l$ then $\arelation_l^*(\aworld_1) = \arelation^*(\aworld_1)$.
By definition of $\avaluation''$,
for every $\aworld_1 \in \arelation(\aworld)$ we then conclude
we have
\begin{nscenter}
$\pair{\aworld}{\aworld_1} \in \arelation_1 \iff \amap(\arelation_1^*(\aworld_1)) \subseteq \avaluation''(\avarpropbis_j)$ \qquad and \qquad $\pair{\aworld}{\aworld_1} \in \arelation_2 \iff \amap(\arelation_2^*(\aworld_1)) \subseteq \avaluation''(\avarpropbis_k)$;
\end{nscenter}
where $\amap(\aset) \egdef \{\amap(x) \mid x \in \aset\}$, for every set $\aset$.
Thus, $\amodel'',\aworld' \models \Box(\avarpropbis_j \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_k)\!\land\!\Box(\avarpropbis_k \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_j)\big)$;
which allows us to conclude that
$\amodel'',\aworld' \models \atranslation_i(\aformula_1 \chopop \aformula_2)$.

\item[($\Leftarrow$):]
Suppose $\amodel',\aworld' \models \atranslation_i(\aformula_1 \chopop \aformula_2)$. Let $j, k \in \interval{1}{3}$ s.t.\ $j < k$ and $j \neq i \neq k$.
By definition,
\begin{nscenter}
$\amodel',\aworld' \models \exists \avarpropbis_j\, \exists \avarpropbis_k
\big(
   [\avarpropbis_i = \avarpropbis_j + \avarpropbis_k]^{\md{\aformula_1 \chopop \aformula_2}}
   \land \atranslation_j(\aformula_1) \land \atranslation_k(\aformula_2)
\land
\Box(\avarpropbis_j \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_k)\!\land\!\Box(\avarpropbis_k \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_j)\big)$.
\end{nscenter}
From the semantics of $\exists \avarpropbis_j \exists \avarpropbis_k \gamma$,
there is a model $\amodel'' = \triple{\worlds'}{\arelation'}{\avaluation''}$ that can be obtained from $\amodel'$ by updating the valuations $\avaluation'(\avarpropbis_j)$ and $\avaluation'(\avarpropbis_k)$ and is such that
\begin{nscenter}
  $\amodel'',\aworld' \models
     [\avarpropbis_i = \avarpropbis_j + \avarpropbis_k]^{\md{\aformula_1 \chopop \aformula_2}}
     \land \atranslation_j(\aformula_1) \land \atranslation_k(\aformula_2)
  \land
  \Box(\avarpropbis_j \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_k)\!\land\!\Box(\avarpropbis_k \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_j)$.
\end{nscenter}
By $\amodel'',\aworld' \models
   [\avarpropbis_i = \avarpropbis_j + \avarpropbis_k]^{\md{\aformula_1 \chopop \aformula_2}}$,
the set of worlds in the set of worlds appearing in $\arelation'|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}}$, i.e. $(\arelation'|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}})^*(\aworld')$, can be \emph{partitioned} into two sets $J$ and $K$ so that $J \subseteq \avaluation''(\avarpropbis_j)$ and $\K \subseteq \avaluation''(\avarpropbis_k)$.
Since $J$ and $K$ partition $(\arelation'|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}})^*(\aworld')$ and $\pair{\amodel''}{\aworld'}$ satisfies
$\Box(\avarpropbis_j \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_k)\!\land\!\Box(\avarpropbis_k \implies \Boxbox^{\md{\aformula_1 \chopop \aformula_2}-1} \lnot \avarpropbis_j)$
we conclude that for every
  $\aworld_1' \in \arelation'(\aworld')$
\begin{nscenter}
  ($\aworld_1' \in J$ implies $(\arelation'|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}-1})^*(\aworld_1') \subseteq J$)
  \qquad
  and
  \qquad
  ($\aworld_1' \in K $ implies $ (\arelation'|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}-1})^*(\aworld_1') \subseteq K$).
  \qquad\qquad\quad \desclabel{($\star$)}{A:msok-label-i}
\end{nscenter}
Now, let us consider $\amodel_1 = \triple{\worlds}{\arelation_1}{\avaluation}$ and $\amodel_2 = \triple{\worlds}{\arelation_2}{\avaluation}$ such that
$\amodel_1 +_{\aworld} \amodel_2 = \amodel$ and
for every
$\aworld_1 \in \arelation(\aworld)$, $\aworld_1 \in \arelation_1(\aworld)$ if and only if $\amap(\aworld_1) \in J$. By \ref{A:msok-label-i} we conclude that
for every $\aworld_1 \in \arelation(\aworld)$
\begin{nscenter}
($\amap(\aworld_1) \in J$ implies
$(\arelation_1|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}-1})^*(\aworld_1) \subseteq \amap^{-1}(J)$)
\qquad
and
\qquad
($\amap(\aworld_1) \in K$ implies
$(\arelation_2|_{\aworld'}^{\leq \md{\aformula_1 \chopop \aformula_2}-1})^*(\aworld_1) \subseteq \amap^{-1}(K)$).
\end{nscenter}
Hence (directly form its definition), $\pair{\amodel''}{\aworld'}$ is a $\pair{\md{\aformula_1 \chopop \aformula_2}}{j}$-encoding of $\pair{\amodel_1}{\aworld}$, as well as a  $\pair{\md{\aformula_1 \chopop \aformula_2}}{k}$-encoding of $\pair{\amodel_2}{\aworld}$.
From $\amodel'',\aworld' \models \atranslation_j(\aformula) \land \atranslation_k(\aformula_2)$, by inductive hypothesis we conclude $\amodel_1,\aworld \models \aformula_1$ and $\amodel_2,\aworld \models \aformula_2$.
Since by definition $\amodel = \amodel_1 +_{\aworld} \amodel_2$, we
have $\amodel,\aworld \models \aformula_1 \chopop \aformula_2$.
\qedhere
\end{description}
\end{proof}


The following result proves \Cref{corr:MSOK-tower}.


\begin{lemma}
  Let $\aformula$ in $\ML(\separate,\chopop)$. Let $\apropsetbis = \{\avarpropbis_1,\avarpropbis_2,\avarpropbis_3\}$ be three atomic propositions not appearing in $\aformula$.
  $\aformula$ is satisfiable w.r.t.\ $\ML(\separate,\chopop)$ if and only if $\atranslation_{1}(\aformula)$ w.r.t.\ satisfiable in $\msokt$.
\end{lemma}


\begin{proof}
\begin{description}
\item[($\Rightarrow$):] Suppose $\aformula$ satisfiable.
Then, consider $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ be a finite forest and $\aworld \in \worlds$ such that $\amodel,\aworld \models \aformula$ (semantics of $\ML(\separate,\chopop)$).
Let $\amodel' = \triple{\worlds'}{\arelation'}{\avaluation'}$ such that
\begin{itemize}
  \item $\arelation' = \arelation|_{\aworld}^{\leq \md{\aformula}}$;
  \item $\worlds' = \pi_1(\arelation') \cup \pi_2(\arelation')$, i.e. $\worlds'$ contains all the worlds appearing in $\arelation'$
        ($\pi_i$ is the projection function on the $i$th component).
  \item $\avaluation'(\avarprop) = \avaluation(\avarprop)$ for every $\avarprop \in \AP \setminus \apropsetbis$. $\avaluation'(\avarpropbis) = \worlds'$ for $\avarpropbis \in \apropsetbis$ (actually, the values for $\avaluation'(\avarpropbis_2)$ and $\avaluation'(\avarpropbis_3)$ can be arbitrary).
\end{itemize}
Directly, $\pair{\amodel'}{\aworld}$ is a $\pair{\md{\aformula}}{1}$-encoding of $\pair{\amodel}{\aworld}$.
By \Cref{A:lemma:MSOK-induction}, $\pair{\amodel'}{\aworld} \models \atranslation_1(\aformula)$ (semantics of $\msokt$).

\item[($\Leftarrow$):] Suppose $\atranslation_1(\aformula)$ satisfiable.
Consider a  finite tree $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ and $\aworld \in \worlds$ such that $\amodel,\aworld \models \atranslation_1(\aformula)$ (semantics of $\msokt$).
By definition,
$\amodel$ is also a finite forest.
It is straightforward to see that  $\pair{\amodel}{\aworld}$ is a $\pair{\md{\aformula}}{1}$-encoding of itself.
Hence, by  \Cref{A:lemma:MSOK-induction}, $\pair{\amodel}{\aworld} \models \aformula$ (semantics of $\ML(\separate,\chopop)$).
\end{description}
\end{proof}


==> proofs/proof-lemma-small-model-bd.tex <==
\begin{proof} The proof is by induction on the modal degree of $\aformula$. The base case with $\md{\aformula} =0$
is by an easy verification as then $\bd{\aformula} = 0$ and therefore satisfaction of $\aformula$ can be witnessed
on a single node model. For the induction step, let us suppose that for all formulae $\aformulabis$ of modal
depth less than $d$, if $\aformulabis$ has a model then it has model in which  each node has at most $\bd{\aformulabis}$ children.

Let $\aformula$ be a satisfiable formula in \GML of modal depth $d+1$.
Let $\maxgmod{\aformula} = \set{\aformulabis_1, \ldots,\aformulabis_n}$ and
$\avarprop_1, \ldots, \avarprop_m$ be
the propositional variables in $\aformula$ that are not in the scope of a graded modality.
We write $\DNF{\aformula}$ to denote the set of formulae in disjunctive normal form
logically equivalent to $\aformula$ with atomic formulae among
$\set{\aformulabis_1, \ldots,\aformulabis_n,\avarprop_1, \ldots, \avarprop_m}$.
We exclude from $\DNF{\aformula}$ the conjunctions and disjunctions with repetitions as well as
conjunctions that do not respect the  conditions below to avoid obvious inconsistencies.
Typically, the conjunctions are of the form  (modulo AC and without repetitions)
$$
\Gdiamond{\geq k_1}{\aformula_1} \wedge \ldots \wedge \Gdiamond{\geq k_m}{\aformula_m}
\wedge
\neg \Gdiamond{\geq k_1'}{\aformula_1'} \wedge \ldots \wedge \neg \Gdiamond{\geq k_m'}{\aformula_{m'}'}
\wedge
\aliteral_1 \wedge \cdots \wedge \aliteral_{m''},
$$
where the $\aliteral_i$'s are literals built over $\avarprop_1, \ldots, \avarprop_m$.  Without loss of generality,
we assume that if $\aformula_i = \aformula'_{j}$, then $k'_j > k_i$ and there are no contradictory
literals in $\aliteral_1 \wedge \cdots \wedge \aliteral_{m''}$.


Let $\aformula' \in \DNF{\aformula}$.
As $\aformula'$ is satisfiable too, there is a conjunction $\aformula''$ in $\aformula'$  that is satisfiable, say of the form below:
$$
\aformula'' =
\Gdiamond{\geq k_1}{\aformula_1} \wedge \ldots \wedge \Gdiamond{\geq k_m}{\aformula_m}
\wedge
\neg \Gdiamond{\geq k_1'}{\aformula_1'} \wedge \ldots \wedge \neg \Gdiamond{\geq k_m'}{\aformula_{m'}'}
\wedge
\aliteral_1 \wedge \cdots \wedge \aliteral_{m''}.
$$
By definition of  $\topbd{\aformula'}$, we have $(k_1 + \cdots + k_m) \leq \topbd{\aformula'} \leq \bd{\aformula}$.
Let $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ be a model and $\aworld \in \worlds$ such that
$\amodel, \aworld \models \aformula''$.
By definition of $\models$, for each $i \in \interval{1}{m}$, there is a set $\aset_i$ made
of $k_i$ children of $\aworld$ such that each child in  $\aset_i$  satisfies $\aformula_i$.
Let  $\amodel' = \triple{\worlds'}{\arelation'}{\avaluation'}$ be the model such that
$\worlds' \egdef \set{\aworld} \cup \set{\aworld' \mid \aworld' \in \arelation^*(\aworld''),
\aworld'' \in \aset_1 \cup \cdots \cup \aset_m}$,
$\arelation' = \arelation \cap (\worlds' \times \worlds')$ and $\avaluation'$ is the restriction of
$\avaluation$ to $\worlds'$. It is easy to verify that $\amodel', \aworld \models
\aformula''$ and $\aworld$ has at most $(k_1 + \cdots + k_m)$ children in $\amodel'$.
By the induction hypothesis, for each $i \in \interval{1}{m}$,
there is a model $\amodel_i = \triple{\worlds_i}{\arelation_i}{\avaluation_i}$ and
$\aworld_i \in \worlds_i$ (say $\pair{\worlds_i}{\arelation_i}$ is rooted at $\aworld_i$)
such that $\amodel_i, \aworld_i \models \aformula_i$ and
each node in $\amodel_i$ has at most $\bd{\aformula_i}$ children.
As $\aformula_i$ is a subformula of $\aformula$, by definition of $\bd{\aformula}$, we have also
$\bd{\aformula_i} \leq \bd{\aformula}$.
Let us build the model $\amodel''$ obtained from $\amodel'$ such that for all $i \in \interval{1}{m}$
and for all children $\aworld' \in \aset_i$, we replace the subtree rooted at $\aworld'$ in $\amodel'$
by a copy of $\amodel_i$. It is then easy to verify that $\amodel'', \aworld \models \aformula''$
and each node in $\amodel''$ has at most $\bd{\aformula}$ children.
This completes the proof for the induction step.
\end{proof}


==> sections/OLD-section-aexppol.tex <==
%!TEX root = ../main.tex

To establish  that \satproblem{\modallogicCC} is in  \aexppol,
given
%% a formula
$\aformula$ in \modallogicCC, we build a logically equivalent formula $\aformula'$ in \GML
 such that the models for $\aformula'$ (if any) do not require a number of children per node
more than exponential in  $\fsize{\aformula}$. The proof
of Theorem~\ref{theorem:clean-cut} needs to be  slightly refined  to improve the way $\aformula'$ is computed.
The \aexppol algorithm consists then in
guessing an exponential-size single tree model and to verify that $\aformula$ holds on its  root, which can be checked
in \aexppol using a standard model-checking algorithm for \MSO (as \modallogicCC can be easily translated into it).

%% BEGIN -- SD 04/01/2020
\cut{
We define below the \defstyle{branching degree} of any formula $\aformula$ in \GML as an upper bound on the number
of children per node in a small model satisfying $\aformula$. Such a branching degree is written $\bd{\aformula}$,
and is defined syntactically.
Let $\aformula$ in \GML be such that $\maxgmod{\aformula} = \set{\Gdiamond{\geq k_1} \aformulabis_1, \ldots, \Gdiamond{\geq k_n}
\aformulabis_n}$.
%%  and
%% the propositional variables not in the scope of a graded modality are $\avarprop_1, \ldots, \avarprop_m$.
We write $\topbd{\aformula}$ to denote  $\max \set{k_i \mid i \in \interval{1}{n}} \times n$
(when  $\maxgmod{\aformula} = \emptyset$, $\topbd{\aformula} \egdef 0$).
(Alternatively, $\topbd{\aformula}$ could be defined more precisely by $k_1 + \cdots + k_n$.)
The \defstyle{branching degree} of any formula $\aformula$ in \GML is defined
as $\bd{\aformula} \egdef \max \set{\topbd{\aformulabis} \mid \aformulabis \in \subf{\aformula}}$,
where $\subf{\aformula}$ is the set of subformulae of $\aformula$.
It is easy to verify that $\bd{\aformula}$ is also equal to $\max (\set{\topbd{\aformula}} \cup
\set{\topbd{\aformulabis} \mid \Gdiamond{\geq k}{\aformulabis} \in \subf{\aformula}})$.
%%
The value $\bd{\aformula}$ reveals to be the relevant measure
to bound the number of children per node.%5
%%


\begin{lemma}
\label{lemma:small-model-bd}
Every satisfiable $\aformula$ in \GML has a model with branching degree at most $\bd{\aformula}$.
\end{lemma}%%
%%
%% Long version
%\input{proofs/proof-lemma-small-model-bd}
%%
Consequently, if $\aformula$ in \GML is satisfiable, then
%% the formula
$\aformula$ has a tree model with at most
$\bd{\aformula}^{d+1}$ worlds, where $d = \md{\aformula}$.
% is the modal degree of $\aformula$ understood
%as the maximal number of imbricated graded modalities in $\aformula$.
}
%% END -- SD 04/01/2020


Below, we introduce the fragment $\sf{F}$ for which its Lemma~\ref{lemma:f-gml}
is essential for the exponential-size model property for \modallogicCC.


 Let us consider the following fragment of \modallogicCC (let us call it $\sf{F}$)
defined by the grammar below:
      \begin{nscenter}
      $
    \aformula::= \Gdiamond{\geq k} \aformulabis \ \mid \ \avarprop \ \mid \
                  \aformula \chopop \aformula  \ \mid \
                  \aformula \wedge \aformula  \ \mid \
                  \neg \aformula,
    $
      \end{nscenter}
    where $\avarprop \in \varprop$ and $\Gdiamond{\geq k} \aformulabis$ is a formula in \GML (abusively
    assumed in \modallogicCC but we have seen that $\GML \preceq \modallogicCC$).
    Given a formula $\aformula$ in \modallogicCC or in $\sf{F}$, we write $\cd{\aformula}$ to denote
    its \defstyle{composition degree}, i.e. the maximal number of imbrications of $\chopop$ in $\aformula$.
    Similarly, we write $\dweight{\aformula}$ to denote
    its \defstyle{diamond weight}, i.e. the  number of distinct subformulae of $\aformula$
    whose outermost connective is a modality $\Diamond$ or $\Gdiamond{\geq k}$.
    Finally, let $\aformula$ be in $\sf{F}$ built over the \GML formulae
    $\set{\Gdiamond{\geq k_1} \aformulater_1, \ldots,
     \Gdiamond{\geq k_n} \aformulater_n}$.
     We write $\newbd{m}{\aformula}$ to denote the value
    $\newbd{m}{\Gdiamond{\geq k_1} \aformulater_1 \wedge \cdots \wedge \Gdiamond{\geq k_n} \aformulater_n}$.
    Indeed, so far $\newbd{m}{\aformulabis}$ were only defined for \GML formulae $\aformulabis$.
    Lemma~\ref{lemma:f-gml} below can be viewed as a generalisation of Lemma~\ref{lemma:f-one},
    essential for forthcoming Lemma~\ref{lemma:small-gml-formula}.

\begin{lemma}
\label{lemma:f-gml}
Let $\aformula$ be 
%% a formula 
in the fragment $\sf{F}$ built over \GML formulae in
$\set{\Gdiamond{\geq k_1} \aformulater_1, \ldots,
     \Gdiamond{\geq k_n} \aformulater_n}$ and $\widehat{k} = \max \set{k_1, \ldots, k_n}$.
There is a \GML
formula $\aformulabis$ such that
\begin{enumerate}
\itemsep 0 cm
\item $\aformula \equiv \aformulabis$; $\md{\aformulabis} \leq \md{\aformula}$,
\item $\newbd{0}{\aformulabis} \leq \widehat{k}  \times 2^{\cd{\aformula}} \times 2^n$;
      $\newbd{1}{\aformulabis} \leq n \times \newbd{1}{\aformula}$,
\item $\newbd{m}{\aformulabis} = \newbd{m}{\aformula}$, for all $m \geq 2$.
\end{enumerate}
\end{lemma}

Consequently, $\maxbd{\aformulabis}$ is at most exponential in $\fsize{\aformula}$.
Applying adequately the transformation from Lemma~\ref{lemma:f-gml} to a formula
in \modallogicCC allows us to get a logically equivalent \GML formula having small models.
%%
%% SD 04/01/20
%%
%% Below, we state the core property that allows us to conclude the  upper
%% bound \aexppol for \satproblem{\modallogicCC}. Its proof is based on a syntactical analysis
%% for the transformations in Section~\ref{section-cc-less-gml}, on Lemma~\ref{lemma:f-gml}
%% and on further refinements to fit the exponential bounds.
%%
%%
\begin{lemma}
\label{lemma:small-gml-formula}
Every satisfiable formula in \modallogicCC has an ex\-po\-nen\-tial-size model.
%%
%% SD 04/01/2020
%%
%% Let $\aformula$ be
%% %% a formula
%% in \modallogicCC. There is
%% %% a formula
%% $\aformula'$ in \GML such that $\aformula \equiv \aformula'$, $\maxbd{\aformula'}$
%% is exponential in $\fsize{\aformula}$.
%%
%%
%% SD 04/01/2020
%%
%%  \leq
%% \fsize{\aformula} \times 2^{\fsize{\aformula}}$.
%%
%% SD: 26/03/2019
%%
%%  and $\aformula'$ can be computed
%% in exponential-time in $\fsize{\aformula}$.
%%
\end{lemma}%%
%%
%% Long version
%\input{proofs/proof-lemma-small-gml-formula}
%%
The proof of~\Cref{lemma:small-gml-formula}
(relying on syntactical analysis
from Section~\ref{section-cc-less-gml} and on Lemma~\ref{lemma:f-gml})
consists in showing that
for all formulae $\aformula$ in  \modallogicCC, there is a logically equivalent formula
$\aformula'$ in \GML such that $\maxbd{\aformula'}$ is exponential in $\fsize{\aformula}$,
which is sufficient by Lemma~\ref{lemma:small-model-newbd} to get the exponential-size model property,
whence the upper bound \aexppol.

\begin{theorem}
\label{theorem:complexity-clean-cut}
\satproblem{\modallogicCC} is  in \aexppol.
\end{theorem}%%
%%

The (standard) proof consists in observing that to check the satisfiability
status of $\aformula$ in \modallogicCC, first guess an exponential-size tree model
(thanks to Lemma~\ref{lemma:small-gml-formula}) and check whether its root satisfies $\aformula$,
which  can be done in exponential-time  using an alternating Turing machine with a linear amount
of alternations (between universal states and existential states)
by viewing \modallogicCC as a fragment of \MSO.


%% SD 07/01/20 -- lack if space
\cut{
\begin{proof} (sketch)  Let $\aformula$ be  in \modallogicCC. Here is the
algorithm running in exponential-time on $\fsize{\aformula}$ with an %ATM
alternating Turing machine using only polynomially
many alternations.
%%  to decide the satisfiability status of $\aformula$.
\begin{enumerate}
\itemsep 0 cm
%% \item By Lemma~\ref{lemma:small-gml-formula}, compute a formula $\aformula'$ in \GML in exponential-time
%% in $\fsize{\aformula}$ such that  $\aformula \equiv \aformula'$ and $\bd{\aformula'} \leq \fsize{\aformula} \times 2^{\fsize{\aformula}}$.
%% So, $\aformula'$ is also of exponential size in $\fsize{\aformula}$.
%%
%% SD 20/04/2019
%% It is important to specify that it is a *tree* model (and not a forest with several trees), as
%% if the number of trees is very large, still it would have satisfy the quantitative  bounds.
%%
\item Guess a {\em tree} model $\amodel = \triple{\worlds}{\arelation}{\avaluation}$
with root $\aworld \in \worlds$,
 whose depth is bounded by $\md{\aformula}$
and of exponential-size thanks to Lemma~\ref{lemma:small-gml-formula}.
%% and each node has at most $\fsize{\aformula} \times 2^{\fsize{\aformula}}$ children. So, $\card{\worlds}$ is in
%% $2^{\mathcal{O}(\fsize{\aformula}^2)}$.
%% Guess $\aworld \in \worlds$.
%(typically $\amodel$ can be restricted to a tree and $\aworld$ is its root)
\item Return the result of checking
%$\aformula$ is satisfiable
$\amodel, \aworld \models \aformula$.
This can be done in exponential-time  using an alternating Turing machine with a linear amount
of alternations (between universal states and existential states).
We can  use a standard model-checking algorithm by viewing \modallogicCC as a fragment of \MSO
and to observe that the number of alternations in the computation is linear in the maximal number of imbrications
of %the composition operator 
$\chopop$ in $\aformula$. \qedhere
\end{enumerate}%%
\end{proof}%%
}



It remains to establish \aexppol-hardness. To do so, we provide a logspace reduction from
the satisfiability problem for the team logic PL[\plcnot] shown \aexppol-complete in~\cite[Theorem 4.9]{HannulaKVV18}.
%%
%% SD 07/01/20 -- lack of space 
%% 
%% (examples of \aexppol-complete quantified propositional logics can be found in~\cite{Hannulaetal16}).
%% 
Let us briefly define PL[\plcnot].
Its formulae  are designed with the grammar
$
\aformula \grammardef\
\avarprop \ \mid \
\plneg \avarprop \ \mid \
\aformula \wedge \aformula \ \mid \
\plcnot \aformula \ \mid \
\aformula \plvee \aformula\,
$,
where $\avarprop$ is a propositional variable from a countably infinite set.
Whereas $\wedge$ and \plcnot \ behave respectively as classical conjunction and classical negation,
the connective $\plneg$ has a negation flavour without being equivalent to
\plcnot and $\plvee$ is actually
a separating connective whose semantics follows. The small dot at the top of $\plneg$ or
$\plvee$ is not originally present in~\cite{HannulaKVV18}: this
is added herein to avoid any confusion with the connectives in \modallogicCC.
Models of PL[\plcnot] are sets of propositional valuations over a finite set of propositional variables,
such sets are called \defstyle{teams} and are denoted below by $\ateam, \ateambis, \ldots$.
A model for a formula $\aformula$ is a team $\ateam$ over a set of propositional variables including
those occurring in $\aformula$ and such that $\ateam \models \aformula$, 
where $\models$ is defined as follows.
%where the satisfaction relation is
%defined as follows.
% \begin{itemize}
% \itemsep 0 cm
% \item $\ateam \models \avarprop$ iff for all $\aplvaluation \in \ateam$, we have $\aplvaluation(\avarprop) = \true$.
% \item $\ateam \models \plneg \avarprop$ iff for all $\aplvaluation \in \ateam$, we have $\aplvaluation(\avarprop) = \false$.
% \item $\ateam \models \aformula_1 \wedge \aformula_2$ iff $\ateam \models \aformula_1$ and
% $\ateam \models \aformula_2$.
% \item $\ateam \models \plcnot \aformula$ iff not $\ateam \models \aformula$.
% \item $\ateam \models \aformula_1 \plvee \aformula_2$ iff there are $\ateambis$ and $\ateambis'$
% such that $\ateam = \ateambis \cup \ateambis'$,   $\ateambis \models \aformula_1$ and $\ateambis' \models \aformula_2$.
% \end{itemize}
\begin{nscenter}
$
\begin{array}{lcl}
\ateam \models \avarprop & \iff & \mbox{for all $\aplvaluation \in \ateam$, we have } \aplvaluation(\avarprop) = \true \\
\ateam \models \plneg \avarprop & \iff & \mbox{for all $\aplvaluation \in \ateam$, we have }\aplvaluation(\avarprop) = \false \\
 \ateam \models \aformula_1 \wedge \aformula_2 & \iff & \ateam \models \aformula_1 \mbox{ and } \ateam \models \aformula_2 \\
\ateam \models \plcnot \aformula & \iff & \ateam \not\models \aformula \\
\ateam \models \aformula_1 \plvee \aformula_2 & \iff & \mbox{there are }\ateambis \mbox{ and }\ateambis' \mbox{ s.t. }\ateam = \ateambis \cup \ateambis', \\   & & \ateambis \models \aformula_1 \mbox{ and } \ateambis' \models \aformula_2.
\end{array}
$
\end{nscenter}
In the clause for handling $\plvee$, the sets $\ateambis$ and $\ateambis'$ are not necessarily disjoint.
%%
%% SD 07/01/2020 -- lack of space
%% 
%% Looking for a team satisfying $\aformula$ requires to consider only propositional variables occurring in $\aformula$,
%% a model for $\aformula$ can be therefore
%% assumed of  exponential size, which allows us easily to obtain the  upper bound \aexppol.
%% 
Now, we show how to design the reduction from the satisfiability problem for  PL[\plcnot]
to the one for \modallogicCC.
Let $\pair{\amodel}{\aworld}$ be a pointed forest, where $\amodel = \triple{\worlds}{\arelation}{\avaluation}$.
An immediate encoding of a team $\ateam$ into $\pair{\amodel}{\aworld}$ consists in having a correspondence
between the propositional valuations in $\ateam$ and the propositional valuations of the children of the current world $\aworld$.
This would work fine if there were no mismatch between the semantics for $\plvee$ (disjointness
not required between the  teams $\ateambis$ and $\ateambis'$), and the one for $\chopop$ (disjointness of the children).
In order to handle this, when checking the satisfaction of $\aformula$ in PL[\plcnot] with $n$ occurrences
of $\plvee$, we impose that,  in $\pair{\amodel}{\aworld}$, if a propositional valuation occurs among
the children of $\aworld$, it occurs initially at least $n+1$ times.
This property must then be maintained after applying $\plvee$ several times, always with respect to the number of occurrences of this operator in the subformula of $\aformula$ that is evaluated.
In this way, non-disjointness of the teams
is encoded by carefully separating the children of $\aworld$ having identical valuations.

Let us now formalise this reduction.
Assume that we wish to translate $\aformula$ from PL[\plcnot],
written with atomic propositions in
$\apropset = \set{\avarprop_1, \dots, \avarprop_m}$.
Suppose that $\aformula$ contains at most $n$ occurrences of the  operator $\plvee$.
We introduce a set
$\apropsetbis = \set{ \avarpropbis_1, \dots, \avarpropbis_{n+1}}$ of
auxiliary propositions, disjoint from $\apropset$ and used in order to distinguish
different copies of the same propositional evaluation of a team.
Hence, with respect to the pointed forest $\pair{\amodel}{\aworld}$,
we require every child of $\aworld$ to satisfy exactly one propositional variable in $\apropsetbis$. This can be done easily, with the following formula:
\begin{nscenter}
  $\tluniq{\apropsetbis} \egdef
  %$$
  % $$
  \Box (\bigwedge_{i \neq i' \in \interval{1}{n+1}} \neg (\avarpropbis_i \wedge \avarpropbis_{i'}) \wedge \bigvee_{i \in \interval{1}{n+1}} \avarpropbis_i).$
\end{nscenter}
Moreover, we require that if a child of $\aworld$ satisfies a propositional valuation over $\avarprop_1, \dots, \avarprop_m$ as well as some $\avarpropbis_{j}$ in $\apropsetbis$, then
there are $n+1$ children satisfying that valuation over $\avarprop_1, \dots, \avarprop_m$, each of them satisfying
a distinct symbol in $\apropsetbis$.
In this way, every valuation over $\avarprop_1,\dots,\avarprop_m$ occurring in some child of $\aworld$,
occurs at least in $n+1$ children of $\aworld$.
However, as the translation the operator  $\plvee$ modifies the set of copies of a propositional evaluation, this property must be extended to arbitrary subsets of $\apropsetbis$. Thus, given $\emptyset \neq \aset \subseteq  \interval{1}{n+1}$,
we require that for every $k \neq k' \in \aset$,
if a children of $\aworld$ satisfies $\avarpropbis_{k}$, then there is child satisfying $\avarpropbis_{k'}$ with the same valuation over $\avarprop_1,\dots,\avarprop_m$. The formula $\tlcopies{\aset}$ defined as
\begin{nscenter}
      $
      \displaystyle\bigwedge_{\mathclap{\quad k \neq k' \in \aset}}\!\!\neg (
      \Box \avarpropbis_{k} \chopop
      (
      \Gdiamond{= 1} \avarpropbis_{k} \wedge
     \neg
     (\true \chopop \Gdiamond{= 1} \avarpropbis_{k} \wedge \Gdiamond{= 1} \avarpropbis_{k'}  \wedge
      \!\bigwedge_{\mathclap{j \in \interval{1}{m}}}\!\!\Diamond \avarprop_j \Rightarrow \Box \avarprop_j
     )
      )
       )
       $
\end{nscenter}
does the job.
Lastly,
before defining the translation map $\atranslation$, we
describe how different copies of the same propositional evaluation are split.
We introduce two auxiliary choice functions $\mathfrak{c}_1$ and $\mathfrak{c}_2$
that take as arguments $\aset \subseteq \interval{1}{n+1}$, and $n_1, n_2 \in \Nat$ with $\card{\aset} \geq n_1 + n_2$ such that
for each $i \in \set{1,2}$, we have $\mathfrak{c}_i(\aset,n_1,n_2) \subseteq \aset$,
$\card{\mathfrak{c}_i(\aset,n_1,n_2)} \geq n_i$. Moreover $\mathfrak{c}_1(\aset,n_1,n_2) \uplus \mathfrak{c}_2(\aset,n_1,n_2) = \aset$.
The maps $\mathfrak{c}_1$ and $\mathfrak{c}_2$ are instrumental to decide how to split
$\aset$ into two disjoint subsets respecting basic cardinality constraints.
The translation map $\atranslation$ is  designed as follows ($\emptyset \neq \aset \subseteq \interval{1}{n+1}$).\\[2pt]
%% $\hphantom{.}\!\atranslation(\avarprop,\aset) \egdef  \Box \avarprop;\hfill  \atranslation(\plneg \avarprop,\aset) \egdef \Box
%% \neg \avarprop; \hfill   \atranslation(\plcnot \aformula,\aset) \egdef \neg  \atranslation(\aformula,\aset);$\\
$\atranslation(\avarprop,\aset) \egdef \Box ((\bigvee_{j \in \aset} \avarpropbis_j) \Rightarrow \avarprop)$\\
$\atranslation(\plneg \avarprop,\aset) \egdef \Box ((\bigvee_{j \in \aset} \avarpropbis_j) \Rightarrow \neg \avarprop),\hfill
\atranslation(\plcnot \aformula,\aset) \egdef \neg  \atranslation(\aformula,\aset)$\\
 $
 \arraycolsep=1.4pt
 \begin{array}{ll}
      \atranslation(\aformula_1 \wedge \aformula_2,\aset) & \egdef\,  \atranslation(\aformula_1,\aset) \wedge \atranslation(\aformula_2,\aset);\\
      \atranslation(\aformula_1 \plvee \aformula_2,\aset) & \egdef\,
      \displaystyle
      (\atranslation(\aformula_1,\aset_1) \land
      %% \Box\! \bigvee_{\mathclap{i \in \aset_1}}\!\avarpropbis_i
      \tlcopies{\aset_1}) \chopop\, (\atranslation(\aformula_2,\aset_2)
      \land
      %% \Box\!\bigvee_{\mathclap{i \in \aset_2}}\!\avarpropbis_i),
       \tlcopies{\aset_2}),
 \end{array}
 $\\[2pt]
% \begin{itemize}
% \itemsep 0 cm
% \item $\atranslation(\avarprop,\aset) \egdef \Box \avarprop$; $\atranslation(\plneg \avarprop,\aset) \egdef \Box \neg \avarprop$;
%       $\atranslation(\plcnot \aformula,\aset) \egdef \neg  \atranslation(\aformula,\aset)$,
% \item $\atranslation(\aformula_1 \wedge \aformula_2,\aset) \egdef \atranslation(\aformula_1,\aset) \wedge \atranslation(\aformula_2,\aset)$,
% \item $\atranslation(\aformula_1 \plvee \aformula_2,\aset) \egdef (\Box(\bigvee_{i \in \aset_1} \avarpropbis_i)  \wedge \atranslation(\aformula_1,\aset_1)) \chopop
% (\Box(\bigvee_{i \in \aset_2} \avarpropbis_i) \wedge \atranslation(\aformula_2,\aset_2))$ where
where
{\bfseries \itshape{(i)}}
$\card{\aset}$ is greater or equal to the number of occurrences of $\plvee$ in $\aformula_1 \plvee \aformula_2$;
{\bfseries \itshape{(ii)}}
given $n_1, n_2$ such that
$n_1$ (resp. $n_2$) is the number of occurrences of $\plvee$ in $\aformula_1$ (resp. $\aformula_2$) plus one,
for each $i \in \set{1,2}$ we have $\mathfrak{c}_i(\aset,n_1,n_2) = \aset_i$.
%\end{itemize}

\Cref{lemma:correctness-PL} below
guarantees that starting with a linear number of children with the same propositional valuation
is sufficient to encode $\plvee$ within \modallogicCC.
%%
%% SD 07/01/20 -- lack of space
%% 
%% ,hence solving the mismatch between the two operators $\plvee$ and $\chopop$\,.
%% 

\begin{lemma}
\label{lemma:correctness-PL}
Let $\aformula$ be in  PL[\plcnot] with $n$ occurrences of  $\plvee$
and built upon $\avarprop_1$, \ldots, $\avarprop_m$. Then, $\aformula$ is satisfiable iff so is
\begin{nscenter}
$
\tluniq{\avarpropbis_1, \ldots,  \avarpropbis_{n+1}} \wedge \tlcopies{\interval{1}{n+1}}
\wedge \atranslation(\aformula, \interval{1}{n+1}).
$
\end{nscenter}
\end{lemma}

The proof of Lemma~\ref{lemma:correctness-PL} is based on the property below.
Let $\pair{\amodel}{\aworld}$ be a pointed forest satisfying $\tluniq{\apropsetbis}$, $\ateam$ be a team  built upon $\apropset$ and
$\emptyset \neq \aset \subseteq \interval{1}{n+1}$. We write $\pair{\amodel}{\aworld} \equiv_{\apropset}^{\aset} \ateam$ iff
the conditions below are satisfied.
\begin{enumerate}
\itemsep 0 cm
\item For all valuations $\aplvaluation \in \ateam$, for all $k \in \aset$, there is $\aworld' \in \arelation(\aworld)$ such that
for all $i \in \interval{1}{n}$, we have $\amodel, \aworld' \models \avarprop_i$ iff $\aplvaluation(\avarprop_i) = \top$ (written $\amodel, \aworld'
\models \aplvaluation$) and $\amodel, \aworld' \models \avarpropbis_{k}$.
\item For all valuations $\aplvaluation$ such that
      (for all $k \in \aset$, there is $\aworld'_{k} \in \arelation(\aworld)$ such that
      $\amodel, \aworld'_k
\models \aplvaluation$ and $\amodel, \aworld'_k
\models \avarpropbis_{k}$), we have $\aplvaluation \in \ateam$.
\end{enumerate}
Hence, when $\pair{\amodel}{\aworld} \equiv_{\apropset}^{\aset} \ateam$, the children of $\aworld$ encodes the team $\ateam$ with the property
that each encoding of $\aplvaluation \in \ateam$ is witnessed by $\card{\aset}$ witness worlds.
One can show that given
 $\pair{\amodel}{\aworld}$  such that $\amodel, \aworld \models \tluniq{\apropsetbis} \wedge \tlcopies{\aset}$
and a team $\ateam$  such that $\pair{\amodel}{\aworld} \equiv_{\apropset}^{\aset} \ateam$,  for all
 $\aformulabis$ such that the number of occurrences of $\plvee$ plus one is at most   $\card{\aset}$, we have
$\ateam \models \aformulabis$ iff $\amodel, \aworld \models \atranslation(\aformulabis, \aset)$.





\cut{
\begin{proof} (sketch) The proof relies on the following properties:
\begin{enumerate}
\item
$\amodel, \aworld \models \tluniq{\avarpropbis_1, \ldots,  \avarpropbis_{n+1}} \wedge \tlcopies{\interval{1}{n+1}}$
iff all the children of $\aworld$ satisfies exactly one propositional variable from
$\set{\avarpropbis_1, \ldots,  \avarpropbis_{n+1}}$ and if a child satisfies one propositional valuation on
$\avarprop_1, \ldots, \avarprop_{m}$, then for each $\avarpropbis_j$, there is a child of $\aworld$
satisfying $\avarpropbis_j$ and that valuation.
\item Let $\ateam$ be a team built upon $\set{\avarprop_1, \ldots, \avarprop_{m}}$,
      $\aset$ be a non-empty subset of $\interval{1}{n+1}$, and $\pair{\amodel}{\aworld}$ be
      such that
      \begin{enumerate}
      \item the set of propositional valuations over $\set{\avarprop_1, \ldots, \avarprop_{m}}$ obtained from the
       children of $\aworld$ is equal to $\ateam$,
      \item all the children of $\aworld$ satisfies exactly one propositional variable from
$\set{\avarpropbis_i  \mid  i \in \aset}$ and if a child satisfies one propositional valuation on
$\avarprop_1, \ldots, \avarprop_{m}$, then for each $\avarpropbis_j$ with $j \in \aset$, there is a child of $\aworld$
satisfying $\avarpropbis_j$ as well as that valuation.
      \end{enumerate}
      For all formulae $\aformula$ in PL[\plcnot] built upon $\set{\avarprop_1, \ldots, \avarprop_{m}}$ and with
      at most $\card{\aset}$ occurrences of $\plvee$, we can show that
      $\ateam \models \aformula$ iff $\amodel, \aworld \models \atranslation(\aformula,\aset)$.\qedhere
\end{enumerate}
\end{proof}
}

Notice that the formula in $\modallogicCC$ involved in \Cref{lemma:correctness-PL} has modal depth $1$.
This is interesting, as by \Cref{theorem:complexity-clean-cut} it implies that
$\satproblem{\modallogicCC}$ is \aexppol-complete even when bounding the modal depth of its formulae (at least to 1). %(as long as it is at least $1$).

\begin{corollary}
      \label{cor:aexpol}
% The satisfiability problem for \modallogicCC is \aexppol-complete.
\satproblem{\modallogicCC} is \aexppol-complete.
\end{corollary}

As we show in the next section, this property does not hold for $\modallogicSC$:
checking for the satisfiability of formulae with modal depth $k$ is exponentially easier than checking for the satisfiability of formulae with modal depth $k+1$.


==> sections/OLD-section-expressive-power-clean-chop.tex <==
%!TEX root = ../main.tex

In order to establish  that \modallogicCC $\preceq$ \GML, %is established constructively
%which essentially amounts to show that
the main property amounts in
showing that \GML is closed under the operator $\chopop$\,, i.e.\ given $\aformula_1$, $\aformula_2$  in \GML, one can construct $\aformulabis$ in \GML such that
$\aformula_1 \chopop \aformula_2 \equiv \aformulabis$.
For instance,
$
(\avarprop \vee \Gdiamond{\geq 3} \avarpropter) \chopop \
(\avarpropbis \vee \Gdiamond{\leq 5} \avarpropbis)
\equiv
(\avarprop \vee \Gdiamond{\geq 3} \avarpropter)
$.
With this property, the general algorithm consists in iteratively replacing innermost subformulae
of the form $\aformula_1 \chopop \aformula_2$ by an equivalent counterpart in \GML, allowing us to eliminate all the occurrences of $\chopop$ and obtain an equivalent formula in \GML.
Notice that the base case will involve subformulae $\aformula_1$ and $\aformula_2$
in \ML (already a fragment of \GML).
%%
%% to construct such $\aformulabis$, consists in replacing an innermost
%% subformula whose main connective is $\chopop$
%% %(say $\aformula_1 \chopop \aformula_2$)
%% by
%% an equivalent formula.
%% % $\aformulabis$.
%%
% but we have seen that \ML can be understood as a fragment of \GML.

%%
%% AM 08/01
%%
% Below, we generalise this translation and we
% identify the core situation to transform $\aformula_1 \chopop \aformula_2$
% into a logically equivalent \GML formula.

%%
%% SD 04/01/2020
%%
%% perform several steps to reduce
%% $\aformula_1 \chopop \aformula_2$, imposing %more and more
%5 conditions
%% on the subformulae $\aformula_1$ and $\aformula_2$ until we reach the core situation to be handled.
%% SD 04/01/2020
%%
%% The construction of $\aformulabis$ from $\aformula_1 \chopop \aformula_2$  witnesses a combinatorial
%% explosion but, by a careful analysis %and by further refinements,
%% we are able to obtain an exponential-size
%% model property that leads to the \aexppol upper bound for \satproblem{\modallogicCC} (see~\Cref{section-aexppol}).
%%

Let us provide a few definitions and notations.
Let $\aformula$ be a formula in \GML. %we write
$\maxpc{\aformula}$ denotes the set of subformulae
$\aformulabis$ of $\aformula$ such that $\aformulabis$ is a maximal modality-free formula (without any occurrence
of a graded modality and one of its occurrences in $\aformula$ does not belong to a larger modality-free subformula).
For instance, $\maxpc{(\avarprop \vee \Gdiamond{\geq 3} \avarpropter) \wedge (\avarpropbis \vee \avarprop)}
= \set{\avarprop, \avarpropbis \vee \avarprop}$.
Similarly, %we write
$\maxgmod{\aformula}$ denotes the set of subformulae
$\aformulabis$ of $\aformula$ such that $\aformulabis$ is of the form $\Gdiamond{\geq k} \aformulabis'$
and one of its occurrences in $\aformula$ is not in the scope of a graded modality.
For instance, $\maxgmod{(\avarprop \vee \Gdiamond{\geq 3} \avarpropter) \wedge (\avarpropbis \vee
\Gdiamond{\geq 5}{\Gdiamond{\geq 2}{\avarpropbis}})}
= \set{\Gdiamond{\geq 3}{\avarpropter}, \Gdiamond{\geq 5}{\Gdiamond{\geq 2}{\avarpropbis}}}$.
So, any formula $\aformula$ in \GML is a Boolean combination of formulae from
 $\maxpc{\aformula} \cup \maxgmod{\aformula}$.
%%
%% SD 04/01/2020
%%
%% We proceed step by step for the construction of the \GML formula which allows us to eliminate all the  occurrences
%% of the connective $\chopop$.
%%
%% SD 04/01/2020
%%
%% In each lemma below, we deal with particular parts of formulae under the scope of $\chopop$.
%%
%% %% Let us start by the propositional part.
Lastly, we say that $\aformula$
is in \defstyle{good shape} whenever the two following conditions hold:
\begin{enumerate}
\item $\maxpc{\aformula} \subseteq \set{\perp,\top}$.
      Consequently, every propositional variable in $\aformula$ occurs
      in the scope of a graded modality;
\item For every two distinct $\Gdiamond{\geq k} \aformulabis$
and $\Gdiamond{\geq k'} \aformulabis'$ in $\maxgmod{\aformula}$,
the conjunction  $\aformulabis \wedge \aformulabis'$ is unsatisfiable.
\end{enumerate}

Let $\aformula_1$ and $\aformula_2$ be \GML formulae.
First, we show that when $\aformula_1 \wedge \aformula_2$ is in good shape, there is a \GML formula $\aformulabis$
such that $\aformula_1 \chopop \aformula_2 \equiv \aformulabis$.
%, and this is the key property for
%the whole entreprise.
%%
%% SD 04/01/2020
%%
%%  Moreover, for all arbitrary \GML formulae $\aformulater_1$
%% and  $\aformulater_2$, we can establish that $\aformulater_1 \chopop \aformulater_2$ is logically equivalent
%% to a finite disjunction of formulae of the form $\aformulater' \chopop \aformulater''$
%% where $\aformulater' \wedge \aformulater''$ is in good shape (see Appendix~\ref{appendix-good-shape}).
%%
%%
%%
%% SD 04/01/2020
%% The next step to construct a \GML formula  $\aformulabis$  logically equivalent
%% to $\aformula_1 \chopop \aformula_2$ is to
To do so, we
take advantage of basic properties of  Presburger arithmetic (\PA), see e.g.~\cite{Presburger29,Haase18}.
Let $\aformula$ be in \GML  such that
$\maxpc{\aformula} \subseteq \set{\true,\false}$ and
$\set{\aformulabis_1, \ldots, \aformulabis_n}$  contains
the set $\set{\aformulabis \mid \Gdiamond{\geq k} \aformulabis \in \maxgmod{\aformula}}$.
Below, the variables $\avariable, \avariablebis, \avariableter, \ldots$, possibly decorated and occurring in formulae,
are interpreted by natural
numbers in $\Nat$. We define formulae in \PA that state constraints about the number of children satisfying
a formula $\aformulabis_j$. The variable $\avariable_j$ is intended to be interpreted as the number of children satisfying
$\aformulabis_j$.
We write $\aformula^{\PA}(\avariable_1, \ldots, \avariable_n)$ to denote the arithmetical formula obtained
from $\aformula$ by replacing every maximal occurrence of $\Gdiamond{\geq k} \aformulabis_j$ by
$\avariable_j \geq k$. For instance, assuming that $\aformula = \Gdiamond{\geq 5}{(\avarprop \wedge \avarpropbis)}
\vee \neg \Gdiamond{\geq 4}{\neg \avarprop}$, the arithmetical formula
$\aformula^{\PA}(\avariable_1,\avariable_2)$ may take the value $\avariable_1 \geq 5 \vee \neg (\avariable_2 \geq 4)$.
Let $\aformula_1, \aformula_2$ be \GML formulae such that
$\aformula_1 \land \aformula_2$ is in good shape and
 $\set{\aformulabis_1, \ldots, \aformulabis_n}$ is equal to
$\set{\aformulabis \mid \Gdiamond{\geq k} \aformulabis \in \maxgmod{\aformula_1 \wedge \aformula_2}}$.
Let $[\aformula_1,\aformula_2]^{\PA}$ be the \PA formula below:
\begin{nscenter}
$
\begin{array}{lcl}
[\aformula_1,\aformula_2]^{\PA} & \egdef & \exists \ \avariablebis_1^1, \avariablebis_1^2, \ldots, \avariablebis_n^1, \avariablebis_n^2
 \ (\bigwedge_{j=1}^{n} \avariable_j = \avariablebis_j^1 + \avariablebis_j^2) \wedge \\
 & & \ \ \ \ \aformula^{\PA}_1(\avariablebis_1^1, \ldots,\avariablebis_n^1) \wedge
\aformula^{\PA}_2(\avariablebis_1^2, \ldots,\avariablebis_n^2).
\end{array}
$
\end{nscenter}
The formula $[\aformula_1,\aformula_2]^{\PA}$  states that there is a way to divide the children in two distinct sets
and each set allows to satisfy $\aformula^{\PA}_1$ or $\aformula^{\PA}_2$, resp.
As \PA admits quantifier elimination~\cite{Presburger29,Cooper72,Reddy&Loveland78},
there is a quantifier-free formula $\aformulater$
%% logically
equivalent to $[\aformula_1,\aformula_2]^{\PA}$ and its free variables
are among $\avariable_1, \ldots, \avariable_n$.
A priori, the atomic formulae of $\aformulater$ may not be of the simple form
$\avariable_j \geq k$ (e.g. `modulo constraints' or constraints of the form $\sum a_i \avariable_j \geq k$
may be involved).
%%
%% could possibly contain `modulo constraints` of the form $\avariable_j \equiv_k \avariable_{j'} + k'$
%% (but this can be easily excluded from the shape of $[\aformula_1,\aformula_2]^{\PA}$)  but more probably it may contain
%% constraints of the form $\avariable_j + \avariable_{j'} \geq k$.
However, if the atomic formulae of $\aformulater$ are restricted to expressions of the form
$\avariable_j \geq k$, then we write $\aformulater^{\GML}$ to denote the \GML formula
obtained from $\aformulater$ by replacing every occurrence of $\avariable_j \geq k$
by $\Gdiamond{\geq k}{\aformulabis_j}$.
%% As we  show below, we deal only with this kind of atomic formulae.


\begin{lemma}
\label{lemma:elimination-three-two}
Let  $\aformula_1$ and $\aformula_2$ be  in \GML such that
$\aformula_1 \wedge \aformula_2$ is in good shape.
%% Let  $\aformula_1$ and $\aformula_2$ be  in \GML such that
%% $\maxpc{\aformula_1 \wedge \aformula_2} \subseteq \set{\true,\false}$.
$[\aformula_1,\aformula_2]^{\PA}$ is equivalet to quantifier-free \PA formula $\aformulater$ whose
atomic formulae are only of the form $\avariable_j \geq k$.
Moreover, $\aformula_1 \chopop \aformula_2 \equiv
\aformulater^{\GML}$ and $\gr{\aformulater^{\GML}} \leq \gr{\aformula_1} + \gr{\aformula_2}$.
\end{lemma}%%
%%
%% Long version
% \input{proofs/proof-lemma-elimination-three-two}
%%
%% RF: 15/04 : keep it for the long version.
%% SD: 17/04 : ok, but we need it for the analysis about the complexity.
%% AM: 18/04 : we need it.
%% Let us see if it needs to ne included in the appendix.
%%
%% Interestingly enough, the formula $\aformulater^{\GML}$ has a graded rank $\gr{\aformulater^{\GML}} \leq \gr{\aformula_1} + \gr{\aformula_2}$.
%%
The bound on $\gr{\aformulater^{\GML}}$ shown in this key lemma is essential to obtain an exponential bound on the smallest model satisfying a formula in
\modallogicCC (see~\Cref{section-aexppol}).
%%
%%
%% SD 04/01/2020
%%
%%
%% \begin{lemma}
%% \label{lemma:elimination-three}
%% Let  $\aformula_1$ and $\aformula_2$ be  in \GML
%% such that $\aformula_1 \wedge \aformula_2$ is in good shape.
%% %%
%% %% s.t.
%% %% $\maxpc{\aformula_1 \wedge \aformula_2}{=}\emptyset$ and
%% %% for all  $\Gdiamond{\geq k} \aformulabis$
%% %% and $\Gdiamond{\geq k'} \aformulabis'$ in $\maxgmod{\aformula_1 \wedge \aformula_2}$  with $\aformulabis \neq \aformulabis'$,
%% %% %% the formula
%% %% $\aformulabis \wedge \aformulabis'$ is unsatisfiable.
%% There is
%%  %% a formula
%% $\aformulabis$ in \GML such that $\aformula_1 \chopop \aformula_2 \equiv \aformulabis$
%% and  $\gr{\aformulabis} \leq \gr{\aformula_1} + \gr{\aformula_2}$.
%% \end{lemma}%%
%% %%
%%
\cut{Thanks to Lemma~\ref{lemma:elimination-three-two} we can show that \GML is closed under the operator $\chopop$ by reducing the occurrences of this operator to formulae in good shape. In particular, we show that given two arbitrary formulae $\aformula_1$ and $\aformula_2$ in \GML, the formula $\aformula_1 \chopop \aformula_2$ is equivalent to a disjunction of formulae of the form $(\aformulabis_1 \chopop \aformulabis_2) \land \aformulater$,
where $\aformulater$ is a Boolean combination of atomic propositions and $\aformulabis_1 \land \aformulabis_2$ is in good shape (hence equivalent to a formula in \GML by \Cref{lemma:elimination-three-two}).
This can be done completely syntactically: atomic propositions are dealt with using tautologies from propositional calculus, whereas to produce $\aformulabis_1$ and $\aformulabis_2$ we mainly rely on the following equivalences:
\begin{description}[align=right,leftmargin=*,labelindent=1.3cm]
  \item[(guess)] \scalebox{0.85}{$\Gdiamond{\geq k}\aformula$ $\equiv$ $\Gdiamond{\geq k}\big((\aformula \land \aformulabis) \lor (\aformula \land \lnot \aformulabis)\big)$}
  \item[(\scalebox{0.8}{$\Gdiamond{\!\geq k}$}\!dist)] \scalebox{0.85}{if $\aformula \land \aformulabis$ is unsat., $\Gdiamond{\geq k}\!(\aformula {\lor} \aformulabis)$ $\equiv$ $ \bigvee_{\!k {=} k_1 {+} k_2}(\Gdiamond{\geq k_1}\!\aformula \,{\land}\, \Gdiamond{\geq k_2}\!\aformulabis)$}
  \item[(\,$\chopop$\,dist)] \scalebox{0.85}{$(\aformula \lor \aformulabis) \chopop \aformulater$
  $\equiv$ $(\aformula \chopop \aformulater) \lor (\aformulabis \chopop \aformulater)$}
\end{description}}

Though Lemma~\ref{lemma:elimination-three-two} is sufficient
to show that given $\aformula_1$ and $\aformula_2$ in \GML, there is
$\aformulabis$ in \GML such that $\aformula_1 \chopop \aformula_2 \equiv \aformulabis$,
we refine this property in Lemma~\ref{lemma:f-one} (using Lemma~\ref{lemma:elimination-three-two}),
preparing the proof for the exponential-size model property for
\modallogicCC. We need to introduce a few more simple notions.
Let $\aformula$ be a \GML formula with
$\maxgmod{\aformula} = \set{\Gdiamond{\geq k_1} \aformulabis_1, \ldots,\Gdiamond{\geq k_n} \aformulabis_n}$.
We write $\newbd{0}{\aformula}$ to denote the value $k_1 + \cdots + k_n$ and for all
$m \geq 0$, we set $\newbd{m+1}{\aformula} \egdef \max \set{\newbd{m}{\aformulabis} \mid  \Gdiamond{\geq k}{\aformulabis}
\in \maxgmod{\aformula}}$. Hence, $\newbd{m}{\aformula}$ can be understood as the maximal
$\newbd{0}{\aformulabis}$ for some subformula $\aformulabis$ occurring at the modal depth $m$ within $\aformula$.
We write $\maxbd{\aformula}$ to denote the value $\max \set{\newbd{m}{\aformula}
\mid  m \in \interval{0}{\md{\aformula}}}$.
% Given $\aformula \in \GML$, we write $\submax{\aformula}$ to denote
% the set $\set{\aformulater \mid \Gdiamond{\geq k} \aformulater \in \maxgmod{\aformula}}$.
The value $\maxbd{\aformula}$ plays a special role as stated in Lemma~\ref{lemma:small-model-newbd}
below.

\begin{lemma}
\label{lemma:small-model-newbd}
Every satisfiable $\aformula$ in \GML is satisfiable in a pointed tree
with at most $\maxbd{\aformula}^{\md{\aformula}+1}$ worlds.
\end{lemma}%%

In order to show that \modallogicCC has the exponential-size model property, we
shall establish that given $\aformula$ in \modallogicCC, there is a logically equivalent
formula $\aformula'$ in \GML such that $\md{\aformula'} \leq \md{\aformula}$ and
$\maxbd{\aformula'}$ is exponential in $\fsize{\aformula}$. Here is a key lemma to do so.

\begin{lemma}
\label{lemma:f-one}
Let $\aformulabis_1$ and $\aformulabis_2$ be two formulae in \GML such that
$\maxgmod{\aformulabis_1} \cup \maxgmod{\aformulabis_2} = \set{\Gdiamond{\geq k_1} \aformulater_1, \ldots,
     \Gdiamond{\geq k_n} \aformulater_n}$ and $\widehat{k} = \max \set{k_1, \ldots, k_n}$.
There is a \GML
formula $\aformulabis$ such that
$\aformulabis\,{\equiv}\,\aformulabis_1 \chopop \aformulabis_2$,
\hfill
$\newbd{0}{\aformulabis}\,{\leq}\, \widehat{k} \, 2^{n+1}$ and
\hfill
$\newbd{1}{\aformulabis}\,{\leq}\, n \, \newbd{1}{\aformulabis_1 {\land} \aformulabis_2}$.
\end{lemma}


%%
%% SD 04/01/20
%% The last property to eliminate $\chopop$ in one step, is stated below.%%
%%
%% The proof is immediate by using
%% Lemma~\ref{lemma:elimination-three-one} (from the technical appendix)
%% and~\Cref{lemma:elimination-three-two}. Finally, by putting all together, we establish that all the occurrences
%% of $\chopop$ can be eliminated.
%% %%
%% \begin{lemma}
%% \label{lemma:elimination-four}
%% Let  $\aformula_1$ and $\aformula_2$ be  in \GML.
%% There is  $\aformulabis$ in \GML such that $\aformula_1 \chopop \aformula_2 \equiv \aformulabis$.
%% \end{lemma}%%
%% %%
%% The proof of~\Cref{lemma:elimination-four} is obtained by applying the translation
%% from~\Cref{lemma:elimination-three,lemma:good-shape} (from Appendix~\ref{appendix-good-shape}
%% stating that we can always restrict ourselves to formulae in good shape).
%% %% as the assumptions of each lemma correspond to the conditions of the translated formula of the previous one.
%% %% For instance,~\Cref{lemma:elimination-one} guarantees $\maxpc{\aformula_1\wedge\aformula_2}=\emptyset$, a
%% %% condition required in the rest of the construction. The fact that formulae that are syntactically different under the scope of a
%% %% graded modality are unsatisfiable is guaranteed by \Cref{lemma:elimination-two}.~\Cref{lemma:elimination-three-two} ensures
%% %% that atomic formulae have the proper shape.
%%
The exponential blow-up in~\Cref{lemma:f-one} is due to the construction of formulae in good shape to be able
to use~\Cref{lemma:elimination-three-two}.
%% SD 07/01/20 -- lack of space
%%
%% Note that~\Cref{lemma:f-one} is reminiscent to~\cite[Lemma 3]{Echenim&Iosif&Peltier19}
%% and~\cite[Lemma 9]{Demri&Fervari&Mansutti19} as it deals with the constructive elimination
%% of a separating connective, though it concerns another logical language and %distinct
%% models.
%%

\begin{theorem}
\label{theorem:clean-cut}
\modallogicCC $\preceq$ \GML. Therefore, $\modallogicCC \approx \GML$.
\end{theorem}
%
%% Long version
%\input{proof-theorem-clean-cut.tex}
%
To prove \modallogicCC $\preceq$ \GML, we apply several times
~\Cref{lemma:f-one} causing each time
a potential exponential blow-up.
%% SD 20/04/2019
%% It is important to add 'each time' because without further analysis this would lead to a non-elementary complexity
%% This is in Section 3.2 that we explain how to tamr the combinatorial explosion
%%
In order to provide an optimal complexity upper bound, we need to tame the combinatorial explosion.%%%%


==> sections/OLD-section-nonelementary-children-SC.tex <==
%!TEX root = ../main.tex

\subsection{Enforcing $\amapter(j,n)$ children.}
Let $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ be a finite forest and ${\aworld} \in \worlds$.
We consider two disjoint sets of atomic propositions $\{\avarprop_1,\dots,\avarprop_n,\treeval\}$ and $\Aux = \{\avariable, \avariablebis, \avarleft, \avarselect, \avarright\}$ (whose role is defined below).
We call $\aaux$-node (resp. $\Aux$-node) a world satisfying the proposition $\aaux \in \Aux$ (resp. satisfying a proposition in $\Aux$). We call instead $\avartree$-node a world that satisfies the formula $\avartree \egdef \bigwedge_{\aaux \in \Aux}  \lnot \aaux$.
Every world of $\amodel$ is either a $\avartree$-node or a $\Aux$-node.
We say that a $\aworld''$ is a $\avartree$-child of $\aworld'$ if $\aworld'' \in \arelation(\aworld')$ and $\aworld''$ is a $\avartree$-node. We define the concepts of $\Aux$-child and $\aaux$-child similarly.

The key development of our reduction is given by the definition of a formula, exponential in $j \geq 1$ and polynomial in $n \geq 1$, that when satisfied by $\pair{\amodel}{\aworld}$ forces every $\avartree$-node in $\arelation^i(\aworld)$, where $0 \leq i < j$, to have exactly $\amapter(j-i,n)$ $\avartree$-children, each of them encoding a different number in $\interval{0}{\amapter(j-i,n)-1}$.
As we impose that $\aworld$ is a $\avartree$-node, it must have $\amapter(j,n)$ $\avartree$-children.
We assume $n$ to be fixed throughout this section and denote this formula simply as $\complete{j}$.
From the property above, notice that if $\amodel,\aworld \models \complete{j}$ then
for every $i \in \interval{1}{j-1}$ and every $\avartree$-node $\aworld' \in \arelation^i(\aworld)$ we have $\amodel,\aworld' \models \complete{j-i}$.

First of, let us informally describe how numbers are encoded in the model $\pair{\amodel}{\aworld}$ satisfying $\complete{j}$. Let $i \in \interval{1}{j}$.
Given a $\avartree$-node $\aworld' \in \arelation^i(\aworld)$, $\nbexp{\aworld'}{i}$ denotes the number encoded by $\aworld'$. We omit the subscript $i$ when it is clear from the context.
When $i = j$,
we represent $\nb{\aworld'}$ by using the truth values
of the atomic propositions $\avarprop_1, \dots, \avarprop_n$.
The proposition variable $\avarprop_b$ is responsible for the $b$-th bit of the number, with the least significant bit being encoded by $\avarprop_1$.
For example, for $n = 3$ we have $\amodel, \aworld' \models \avarprop_3 \land \avarprop_2 \land \lnot \avarprop_1$ whenever $\nb{\aworld'} = 6$.
The formula $\complete{1}$ forces the parent of $\aworld'$ (i.e.\ a $\avartree$-node in $\arelation^{i-1}(\aworld)$)
to have exactly $2^n$ $\avartree$-children by requiring one $\avartree$-child for each possible
valuation upon  $\avarprop_1,\dots,\avarprop_n$.
Otherwise, for $i < j$ (and therefore $j \geq 2$), the number $\nbexp{\aworld'}{i}$ is represented by
the binary encoding of the truth values of $\treeval$ on the $\avartree$-children of $\aworld'$ which, since $\pair{\amodel}{\aworld'} \models \complete{j-i}$, are $\amapter(j-i,n)$ children implicitly ordered by the number they, in turn, encode.
The essential property of $\complete{j}$ is therefore the following: given a $\avartree$-node $\aworld'' \in \arelation^i(\aworld)$ in the numbers encoded by its $\avartree$-children represent positions in the binary representation of the number $\nbexp{\aworld''}{i}$.
It is thanks to this property that the formula $\complete{j}$
forces $\aworld$ to have exactly $2^{\amapter(j-1,n)}$ children, all encoding different numbers in $\interval{0}{\amapter(j,n)-1}$.
This is roughly represented in Figure~\ref{figure-type-j},
where $``1"$ stands for $\treeval$ being true whereas $``0"$ stands for $\treeval$ being false.
\begin{figure}
\begin{tikzpicture}
  \node (upleft) at (0,0) {};

  \path (upleft.center) -- ++(0.38\linewidth,-0.4) node[dot,label={$\aworld$}] (root) {.};

  \draw[pto] (root.center) -- ++ (-0.26\linewidth,-1) node[dot] (l1) {};
  \draw[pto] (root.center) -- ++ (0.09\linewidth,-1) node[dot] (c1) {};
  \draw[pto] (root.center) -- ++ (0.39\linewidth,-1) node[dot] (r1) {};

  \path (root.center) -- ++ (-0.086\linewidth,-1.2) node (dots) {$\scaleobj{1.8}{\dots}$};

  \foreach \x in {l1,c1,r1} {
    \draw[pto] (\x.center) -- ++ (-0.08\linewidth,-1.2) node[dot] (l\x) {};
    \draw[pto] (\x.center) -- ++ (0.03\linewidth,-1.2) node[dot] (c\x) {};
    \draw[pto] (\x.center) -- ++ (0.117\linewidth,-1.2) node[dot] (r\x) {};

      \path (\x.center) -- ++ (-0.024\linewidth,-1.2) node (dots) {$\scaleobj{1.1}{\dots}$};


      \path (\x.center) -- ++ (0.08\linewidth,-1.6) node (min2\x) {$\scaleobj{0.9}{<}$};

      \path (\x.center) -- ++ (-0.024\linewidth,-1.6) node (min\x) {$\scaleobj{0.9}{<}$};

    \foreach \y in {l,c,r}{
      \path (\y\x.center) -- ++ (-0.024\linewidth,-0.8) node (e1\y\x) {};
      \path (\y\x.center) -- ++ (0.035\linewidth,-0.8) node (e2\y\x) {};

      \draw[gray!80,fill=gray!80] (\y\x.center) -- (e1\y\x.center) -- (e2\y\x.center) -- (\y\x.center);
      \draw[alin] (\y\x.center) -- (e1\y\x.center);
      \draw[alin] (\y\x.center) -- (e2\y\x.center);
    }
  }

  \node[label={$1$}] at (ll1) {};
  \node[label={[xshift=1pt]$1$}] at (cl1) {};
  \node[label={$1$}] at (rl1) {};

  \node[label={$0$}] at (lc1) {};
  \node[label={[xshift=1pt]$0$}] at (cc1) {};
  \node[label={$1$}] at (rc1) {};

  \node[label={$0$}] at (lr1) {};
  \node[label={[xshift=1pt]$0$}] at (cr1) {};
  \node[label={$0$}] at (rr1) {};

  \path (upleft) -- ++(\linewidth,0) node[label={[xshift=-46pt,yshift=-16pt]$\scaleobj{0.8}{\complete{j}, \text{ has } \amapter(j,n) \text{ children}}$}] (upright) {};
  \path let \p1 = (e1ll1) in (upleft) -- ++ (0,\y1) node (bottomleft) {};
  \path let \p1 = (e1ll1) in (upright) -- ++ (0,\y1) node (bottomright) {};

  \path (upleft) -- ++ (0,-1.3) node (midleft) {};
  \path (upright) -- ++ (0,-1.3) node[label={[xshift=-17pt,yshift=-16pt]$\scaleobj{0.8}{\complete{j{-}1}}$}] (midright) {};

  \path (midleft) -- ++ (0,-1.2) node (downleft) {};
  \path (midright) -- ++ (0,-1.2) node[label={[xshift=-13pt,yshift=-13pt]$\scaleobj{0.6}{\complete{j{-}2}}$}] (downright) {};

  \begin{pgfonlayer}{bg0}

    \draw[gray!5,fill=gray!5] (upleft.center) -- (bottomleft.center) -- (bottomright.center) -- (upright.center) -- (upleft.center);


    \draw[gray!25,fill=gray!25] (midleft.center) -- (bottomleft.center) -- (bottomright.center) -- (midright.center) -- (midleft.center);


    \draw[gray!50,fill=gray!50] (downleft.center) -- (bottomleft.center) -- (bottomright.center) -- (downright.center) -- (downleft.center);

  \end{pgfonlayer}

\end{tikzpicture}
\caption{Schema of a model satisfying $\complete{j}$\hfill (for $j \geq 2$).}\label{figure-type-j}
\end{figure}

To characterise these trees in \modallogicSC we simulate second-order quantification by using $\Aux$-nodes.
Informally, we require a pointed forest $\pair{\amodel}{\aworld}$ satisfying $\complete{j}$ to be s.t.\
\begin{itemize}
\item every $\avartree$-node $\aworld' \in \arelation(\aworld)$ has exactly one $\avariable$-children, and one (different) $\avariablebis$-children. These nodes do not satisfy any other auxiliary propositions;
\item for every $i \geq 2$, every $\avartree$-node $\aworld' \in \arelation^i(\aworld)$ has exactly five $\Aux$-children, each satisfying a different auxiliary proposition from $\Aux$.
\end{itemize}
We can simulate second-order existential quantification on $\avartree$-nodes with respect to the symbol $\aaux \in \Aux$
by using the  operator $\separate$ in order to remove edges leading to $\aaux$-nodes. We then evaluate whether a property holds
on the resulting model where a $\avartree$-node ``satisfies'' $\aaux \in \Aux$ if it has a child satisfying $\aaux$.
To better show the complementary roles that $\avartree$-nodes and $\Aux$-nodes have in the reduction, given a formula $\aformula$ we write
$\HMDiamond{\avartree} \aformula$ for the formula $\Diamond (\avartree \land \aformula)$. This formula is a relativised version of $\Diamond$
that only considers $\avartree$-nodes. Dually, $\HMBox{\avartree} \aformula \egdef \Diamond (\avartree \implies \aformula)$. $\HMDiamond{\avartree}^i$
and $\HMBox{\avartree}^i$ are also defined, as expected.

Let us start to formalise this encoding. Let $j \geq 1$.
First, we restrict ourselves to models where every $\Aux$-node reachable in at most $j$ steps has no children and only satisfy one proposition in $\Aux$, whereas every $\avartree$-node reachable in at most $j$ steps does not have two $\Aux$-children satisfying the same proposition. We express this condition with the formula $\init{j}$, defined as follows:
\[
\Boxbox^{j} \bigwedge_{\mathclap{\aaux \in \Aux}}
\Big(
  \big(
    \avartree \implies \lnot (\Diamond \aaux \separate \Diamond \aaux)
  \big)
\land
  \big(
    \aaux \implies \Box \bottom \land \bigwedge_{\mathclap{\aauxbis \in \Aux \setminus\{\aaux\}}} \lnot \aauxbis
  \big)
 \Big)
\]
where $\Boxbox^0\aformula \egdef \aformula$ and $\Boxbox^{n+1}\aformula \egdef \aformula \land \Box\Boxbox^{n}(\aformula)$.
Notice that the satisfiability of $\init{j}$ is monotonous w.r.t.\ submodels: if $\amodel,\aworld \models \init{j}$ and $\amodel' \sqsubseteq \amodel$ then $\amodel',\aworld \models \init{j}$.

Among the models satisfying $\init{j}$, we characterise the ones that satisfy $\complete{j}$ to be $\pair{\triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ such that
\begin{description}
  \item[\desclabel{(\apS$_j$)}{prop:apS}\phantomlabel{(\apS$_1$)}{prop:apS_1}\phantomlabel{(\apS$_k$)}{prop:apS_k}]
    every $\avartree$-node in $\arelation(\aworld)$ satisfies $\complete{j-1}$;
  \item[\desclabel{(\apZ$_j$)}{prop:apZ}\phantomlabel{(\apZ$_1$)}{prop:apZ_1}]
    there is a $\avartree$-node $\tilde\aworld{\in}\,\arelation(\aworld)$ s.t.\ $\nb{\tilde\aworld} = 0$;
  \item[\desclabel{(\apU$_j$)}{prop:apU}\phantomlabel{(\apU$_1$)}{prop:apU_1}] distinct $\avartree$-nodes in $\arelation(\aworld)$ encode different numbers;
  \item[\desclabel{(\apC$_j$)}{prop:apC}\phantomlabel{(\apC$_1$)}{prop:apC_1}] for every $\avartree$-node $\aworld_1 \in \arelation(\aworld)$, if $\nb{\aworld_1} < \amapter(j,n)-1$ then $\nb{\aworld_2} = \nb{\aworld_1}+1$ for some $\avartree$-node $\aworld_2 \in \arelation(\aworld)$;
  \item[\desclabel{(\apA)}{prop:apA}] $\aworld$ is a $\avartree$-node, every $\avartree$-node in $\arelation(\aworld)$ has one $\avariable$-child and one $\avariablebis$-child, and every $\avartree$-node in $\arelation^2(\aworld)$ has three children satisfying $\avarleft$, $\avarright$ and $\avarselect$, respectively.
\end{description}
For $j \geq 1$, the formula $\complete{j}$ is then defined as
\[
\complete{j} \egdef \pS{j} \land \pZ{j} \land \pU{j} \land \pC{j} \land \pA,
\]
where each conjunct expresses the homonymous property above.
For technical reasons, we also define $\complete{0}$ as $\true$.
The formulae for $\pS{j}$ and $\pA$ can be easily defined as
\begin{align*}
\pS{j} \egdef &\, \HMBox{\avartree}\complete{j-1}\\
\pA \egdef &\, \avartree \land \HMBox{\avartree}(\Diamond \avariable \separate \Diamond \avariablebis) \land \HMBox{\avartree}^2(\Diamond \avarleft \separate \Diamond \avarselect \separate \Diamond \avarright).
\end{align*}
Following the informal description on how numbers are encoded by worlds in $\worlds$, we can also easily define $\pZ{j}$:
\begin{nscenter}
$\pZ{1} \egdef \HMDiamond{\avartree}\!\bigwedge_{b \in \interval{1}{n}} \lnot \avarprop_b$,
\hfill
$\pZ{j} \egdef \HMDiamond{\avartree} \HMBox{\avartree} \lnot \treeval$
\hfill ($j \geq 2$)
\end{nscenter}

The challenge is therefore how to express $\pU{j}$ and $\pC{j}$, the two conditions that, with $\pZ{j}$, guarantee that the number of children of $\aworld$ span all over $\interval{0}{\amapter(j,n)-1}$.

A key point of $\complete{j}$ is that it allows us to manipulate the accessibility relation
in a controlled way when using the  operator $\separate$.
Indeed, let $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ and suppose $\amodel,\aworld \models \init{j} \land \complete{j}$, for $j \geq 1$.
Consider two finite forest models $\amodel_1$ and $\amodel_2$ such that $\amodel_1 + \amodel_2 = \amodel$,
$\amodel_1,\aworld \models \Box \bottom$ and $\amodel_2,\aworld \models \pS{j} \land \pA$.
We can conclude that, among the edges $\pair{\aworld'}{\aworld''} \in \arelation$ appearing in the subtree of depth $j$ rooted at $\aworld$, the structure $\amodel_1$ can only contain the ones such that $\aworld' \in \arelation(\aworld)$ and $\aworld''$ is a $\{\avarleft,\avarselect,\avarright\}$-node.
In particular, every $\avartree$-nodes $\tilde\aworld \in \arelation^i(\aworld)$ ($i \in \interval{0}{j}$)
must still be reachable from $\aworld$ in $\amodel_2$, which implies that the number $\nb{\tilde\aworld}$ encoded by $\tilde\aworld$ is the same in both structures.
This robustness against the unpleasant side-effects of the $\separate$ operator, i.e.\ the general inability to track which edges are lost when considering a submodel, is fundamental in order to reduce $\tiling_k$.

\paragraph{Auxiliary formulae: nominals, forks, $<$ and $+1$.}
In order to define the formulae $\pU{j}$ and $\pC{j}$ (hence completing the definition of $\complete{j}$) we introduce a set of auxiliary formulae, whose semantics is here explained.
These formulae characterise classes of models that emerge quite naturally when trying to capture the semantics of \ref{prop:apU} and \ref{prop:apC}.

As usual, consider a finite forest $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ and a world $\aworld \in \worlds$.
A first ingredient is given by the concept of \emph{local nominals}, borrowed from~\cite{Bednarczyk&Demri19}.
We say that $\aaux \in \Aux$ is a (local) nominal for the depth $i \geq 1$ if there is exactly one $\avartree$-node $\aworld' \in \arelation^i(\aworld)$ having a $\aaux$-child.
The following formula states that $\aaux$ is a local nominal for the depth $i$:
\[
\begin{aligned}
\nominal{\aaux}{i} \egdef
  \HMDiamond{\avartree}^i\Diamond\aaux \land
  {\bigwedge_{\mathclap{k \in \interval{0}{i-1}}}} \HMBox{\avartree}^k \lnot \big(\HMDiamond{\avartree}^{i-k}\Diamond\aaux \separate \HMDiamond{\avartree}^{i-k}\Diamond \aaux\big)
\end{aligned}
\]
We then define the formula $\atnom{\aaux}{i} \aformula \egdef \HMDiamond{\avartree}^i(\Diamond \aaux \land \aformula)$ which, under the hypothesis that $\aaux$ is a nominal for the depth $i$, states that $\aformula$ holds on the $\avartree$-node corresponding to this nominal.
Moreover, we define the formula
$\twonoms{\aaux}{\aauxbis}{i} \egdef \nominal{\aaux}{i} \land \nominal{\aauxbis}{i} \land \lnot \atnom{\aaux}{i} \Diamond \aauxbis$,
which states that $\aaux$ and $\aauxbis$ are two nominals for the depth $i$, corresponding to two distinct worlds.

A second ingredient is given by \emph{forks}: a set of classes of models that naturally emerge when trying to compare the numbers $\nb{\aworld_1}$ and $\nb{\aworld_2}$ of two worlds $\aworld_1,\aworld_2 \in \arelation^i(\aworld)$ (e.g. when checking if $\nb{\aworld_1} = \nb{\aworld_2}$ or $\nb{\aworld_2} = \nb{\aworld_1}+1$ hold).
Given $j \geq i \geq 1$
we introduce the formula $\fork{\aaux}{\aauxbis}{i}{j}$
which is satisfied by $\pair{\amodel}{\aworld}$ if and only if
\begin{itemize}
  \item $\aworld$ has exactly two $\avartree$-children and exactly two paths of $\avartree$-nodes, both of length $i$.
  \item One of these two paths ends on a world (say $\aworld_1$) corresponding to the nominal $\aaux$ whereas the other ends on a world (say $\aworld_2$) corresponding to the nominal $\aauxbis$.
  \item If $i < j$, $\pair{\amodel}{\aworld_1}$ and $\pair{\amodel}{\aworld_2}$ satisfy
  \begin{nscenter}
  $\completeplus{j - i} \egdef \complete{j - i} \land \HMBox{\avartree}(\Diamond \avarleft \land \Diamond \avarselect \land \Diamond \avarright)$.
  \end{nscenter}
\end{itemize}
It should be noted that the worlds in the two paths leading to the worlds corresponding to $\aaux$ and $\aauxbis$ can have $\Aux$-children.
Figure~\ref{figure-fork} schematise a model satisfying $\fork{\aaux}{\aauxbis}{i}{j}$.
\begin{figure}
\begin{tikzpicture}
  \node[dot,label={[yshift=12pt]$\scaleobj{0.8}{\fork{\aaux}{\aauxbis}{i}{j}}$}] (root) at (0,0) {.};
  \path
   (root.center) -- ++(-0.3,0) node (lab) {$\aworld$};

  \draw[pto] (root.center) -- ++(0.16\linewidth,0.7) node[dot] (up) {};
  \draw[pto] (root.center) -- ++(0.16\linewidth,-0.7) node[dot] (down) {};

  \foreach \x in {up,down} {
    \draw[pto] (\x.center) -- ++(0.1\linewidth,0) node[dot] (o\x) {};

    \draw[path] (o\x.center) -- ++(0.16\linewidth,0) node[dot] (t\x) {};

    \draw[pto] (t\x.center) -- ++(0.1\linewidth,0) node[dot,label={right:$\ \ \,\scaleobj{0.8}{\completeplus{j{-}i}}$}] (f\x) {};

    \path (f\x.center) -- ++(0.22\linewidth,0.62) node (up\x) {};
    \path (f\x.center) -- ++(0.22\linewidth,-0.62) node (down\x) {};

    \begin{pgfonlayer}{bg0}
      \draw[gray!15,fill=gray!15] (f\x.center) -- (up\x.center) -- (down\x.center) -- (f\x.center);
      \draw[alin] (f\x.center) -- (up\x.center);
      \draw[alin] (f\x.center) -- (down\x.center);
    \end{pgfonlayer}
  }

  \draw[aux] (fup) -- ++(0,0.38) node[label={[yshift=-5pt]$\aaux$}] (aaux) {};
  \draw[aux] (fdown) -- ++(0,0.38) node[label={[yshift=-5pt]$\aauxbis$}] (aauxbis) {};

  \path (root.center) -- ++(0,-1.1) node (bottomline) {};

  \path let \p1 = (fdown) in (bottomline) -- ++ (\x1,0) node (end) {};

  \draw[segment] (bottomline.center) -- (end.center) node [midway, fill=white] {$i$};

\end{tikzpicture}
\caption{Shape of a model satisfying $\fork{\aaux}{\aauxbis}{i}{j}$.}\label{figure-fork}
\end{figure}

\noindent Since the definition of $\fork{\aaux}{\aauxbis}{i}{j}$ is recursive on $i$ and $j$ (due to $\complete{j-i}$), we postpone the formal definition of this formula to the next two section, where we
treat the base cases for $i = j$ and the inductive case for $j > i$ separately.

The last two formulae are $\less{\aaux}{\aauxbis}{i}{j}$
and $\successor{\aaux}{\aauxbis}{j}$. Under the hypothesis that $\pair{\amodel}{\aworld}$
satisfies $\fork{\aaux}{\aauxbis}{i}{j}$, the formula $\less{\aaux}{\aauxbis}{i}{j}$
is satisfied whenever the two (distinct) worlds $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation^i(\aworld)$ corresponding to the nominals $\aaux$ and $\aauxbis$ are such that $\nb{\aworld_{\aaux}} < \nb{\aworld_{\aauxbis}}$.
Similarly, under the hypothesis that $\pair{\amodel}{\aworld}$
satisfies $\fork{\aaux}{\aauxbis}{1}{j}$, the formula $\successor{\aaux}{\aauxbis}{j}$
is satisfied whenever $\nb{\aworld_{\aauxbis}} = \nb{\aworld_{\aaux}}+1$ holds.
Both this formulae are recursively defined, with base cases for $i = j$ and $j = 1$, respectively.

We now explicit all these recursive formulae: for the base case, we define the formulae  $\fork{\aaux}{\aauxbis}{j}{j}$ and $\less{\aaux}{\aauxbis}{j}{j}$ (for arbitrary $j$), as well as $\successor{\aaux}{\aauxbis}{1}$. From these formulae we are then able to define $\pU{1}$ and $\pC{1}$, which complete the characterisation of $\complete{1}$ and $\completeplus{1}$.
Afterwards, we consider the case $1 \leq i < j$ and $j \geq 2$, and define $\fork{\aaux}{\aauxbis}{i}{j}$, $\less{\aaux}{\aauxbis}{i}{j}$ and $\successor{\aaux}{\aauxbis}{j}$, as well as $\pU{j}$ and $\pC{j}$,
by only relying on formulae that are already defined (by inductive reasoning).
% $\type{j'}$, $\successor{\avariable}{\avariablebis}{j'}$ (where $j' < j$),
% $\fork{\aaux}{\aauxbis}{i'}{j'}$ and $\less{\avariable}{\avariablebis}{i'}{j'}$ (where $j' < j$ or $j' = j$ and $j' - i' < j - i$).

\paragraph{Base cases: $i = j$ / $j = 1$.}
In the following, we consider a finite forest model $\amodel = \triple{\worlds}{\arelation}{\avaluation}$ and a world $\aworld$. As already stated, we are interested in defining the formulae:
\begin{nscenter}
\hfill $\fork{\aaux}{\aauxbis}{j}{j}$,
\hfill $\less{\aaux}{\aauxbis}{j}{j}$,
\hfill $\successor{\aaux}{\aauxbis}{1}$, \hfill\,\\
\hfill $\pU{1}$,
\hfill $\pC{1}$,
\hfill $\complete{1}$. \hfill\,
\end{nscenter}

\noindent Following its informal description, we have
\[
\begin{aligned}
    \fork{\aaux}{\aauxbis}{j}{j} \egdef \Diamond_{=2} \avartree\,
    {\land}\,\HMBox{\avartree}\Boxbox^{j-2}\!(\avartree{\implies}\Diamond_{=1} \avartree)\,
    {\land}\,\twonoms{\aaux}{\aauxbis}{j}\,
\end{aligned}
\]
where we extend the definition of $\Boxbox^j \aformula$ to be $\true$ for $j < 0$.
As previously explained, in the base case, the number $\nb{\aworld'}$ encoded by a $\avartree$-node $\aworld' \in \arelation^{j}(\aworld)$ is represented by the truthiness of the propositional symbols $\avarprop_1,\dots,\avarprop_n$.
Then, the formula $\less{\aaux}{\aauxbis}{j}{j}$ can be defined as
\[
\begin{aligned}
  \less{\aaux}{\aauxbis}{j}{j} \egdef
    {\bigvee_{\mathclap{u \in \interval{1}{n}}}}
      \big(&
        \atnom{\aaux}{j}\lnot \avarprop_u
        \land \atnom{\aauxbis}{j} \avarprop_u \land\!\!{\bigwedge_{\mathclap{v \in \interval{u+1}{n}}}}
        (\atnom{\aaux}{j} \avarprop_v \iff  \atnom{\aauxbis}{j} \avarprop_v)
      \big)
\end{aligned}
\]
As expected, under the hypothesis
$\pair{\amodel}{\aworld} \models \fork{\aaux}{\aauxbis}{j}{j}$, this formula
states that the distinct $\avartree$-nodes $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation^j(\aworld)$ corresponding to $\aaux$ and $\aauxbis$ are s.t.\ $\nb{\aworld_{\aaux}} < \nb{\aworld_{\aauxbis}}$. The definition of this formula uses standard properties about numbers encoded in binary representation with $n$ bits (where the least significant bit is represented by the truth value of $\avarprop_1$).
In particular, it states that there is a bit (encoded by $\avarprop_u$) which is set to $0$ in the binary encoding of $\nb{\aworld_{\aaux}}$ but is set to $1$ in the binary encoding of $\nb{\aworld_{\aauxbis}}$, whereas every the successive bit (encoded by $\avarprop_v$ with $v > u$)
is set to $1$ in $\nb{\aworld_{\aaux}}$ if and only if it is set to $1$ also in $\nb{\aworld_{\aauxbis}}$.

The formula $\successor{\aaux}{\aauxbis}{1}$ uses similar arithmetical properties. It is defined as
\[
    {\bigvee_{\mathclap{\quad u \in \interval{1}{n}}}}
      \!\!\big(
        \atnom{\aaux}{1}(\lnot \avarprop_u {\land}\!\!\bigwedge_{\mathclap{v \in \interval{1}{u-1}}}\!\avarprop_v)
        \land
        \atnom{\aauxbis}{1} (\avarprop_u {\land}\!\!\bigwedge_{\mathclap{v \in \interval{1}{u-1}}}\!\!\lnot \avarprop_v)
        {\land}\!
        {\bigwedge_{\mathclap{\quad \quad v \in \interval{u+1}{n}}}}\!
        (\atnom{\aaux}{1} \avarprop_v\,{\iff}\,\atnom{\aauxbis}{1} \avarprop_v)
      \big)
\]
Under the hypothesis
$\pair{\amodel}{\aworld} \models \fork{\aaux}{\aauxbis}{1}{1}$, this formula
states that the two distinct $\avartree$-nodes $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation(\aworld)$ corresponding to $\aaux$ and $\aauxbis$ are s.t.\ $\nb{\aworld_{\aauxbis}} = \nb{\aworld_{\aaux}}+1$.
As was the case for $\less{\aaux}{\aauxbis}{j}{j}$, this formula state that there must be a bit (encoded by $\avarprop_u$) which is set to $0$ in the binary encoding of $\nb{\aworld_{\aaux}}$ but is set to $1$ in the binary encoding of $\nb{\aworld_{\aauxbis}}$, and that
every the successive bit (encoded by $\avarprop_v$ with $v > u$)
is set to $1$ in $\nb{\aworld_{\aaux}}$ if and only if it is set to $1$ also in $\nb{\aworld_{\aauxbis}}$.
However, differently from $\less{\aaux}{\aauxbis}{j}{j}$, this formula also require that every previous bit of (encoded by $\avarprop_v$ with $v < u$) is set to $1$ in the binary encoding of $\nb{\aworld_{\aaux}}$ but is set to $0$ in the binary encoding of $\nb{\aworld_{\aauxbis}}$.

In order to define $\pU{1}$ we first need to recall that a model satisfying $\complete{1}$ satisfies the formula $\pA$ and hence every $\avartree$-node in $\arelation(\aworld)$ has two auxiliary children, one $\avariable$-node and one $\avariablebis$-node.
The idea is then to use these two children and rely on the $\separate$ operator to state that it is not possible to find a submodel of $\amodel$ such that $\aworld$ only has two distinct children $\aworld_{\avariable}$ and $\aworld_{\avariablebis}$ that correspond to the nominals $\avariable$ and $\avariablebis$, respectively,
and are
such that $\nb{\aworld_\avariable} = \nb{\aworld_\avariablebis}$.
Notice that, in a sense, the $\separate$ is here used to simulate a second-order quantification on $\avariable$ and $\avariablebis$.
Here is the corresponding formula:
\[
\pU{1} \egdef \lnot \big(\true \separate (\fork{\avariable}{\avariablebis}{1}{1} \land \equivalent{\avariable}{\avariablebis}{1}{1})\big)
\]
where, $\equivalent{\avariable}{\avariablebis}{1}{1}$ stands for
$\lnot (\less{\avariable}{\avariablebis}{1}{1} \lor \less{\avariablebis}{\avariable}{1}{1})$.

Let us now consider $\pC{1}$. As done for $\pU{1}$, we rely on the auxiliary propositions $\avariable$ and $\avariablebis$ and use the $\separate$ operator in order to simulate a second-order quantification.
We state that it is not possible to find a submodel of $\amodel$ that looses $\avariable$-nodes from $\arelation^2(\aworld)$, keeps all $\avariablebis$-nodes, and is s.t.\
\begin{itemize}
\item $\avariable$ is a local nominal for the depth $1$, corresponding to a world $\aworld_{\avariable}$ encoding $\nb{\aworld_{\avariable}} < 2^n-1$;
\item it does not exists a submodel where $\aworld$ that has two $\avartree$-children, $\aworld_{\avariable}$ and a second
world $\aworld_{\avariablebis}$, such that $\aworld_{\avariablebis}$ corresponds to the nominal $\avariablebis$
and $\nb{\aworld_{\avariablebis}} = \nb{\aworld_{\avariable}}{+}1$.
\end{itemize}
Thus, we define $\pC{1}$ as follows:
\[
\lnot
  \big(\Box \bottom \separate
    \big(
      \HMBox{\avartree}\Diamond \avariablebis \land \atnom{\avariable}{1} \lnot \one_{1} \land \lnot ( \true \separate (\fork{\avariable}{\avariablebis}{1}{1} \land \successor{\avariable}{\avariablebis}{1}))
    \big)
  \big).
\]
The  subscript ``$1$'' in the formulae $\one_{1}$ refers to the fact that we are treating the base case of $\pC{j}$ with $j = 1$.
We have $\one_{1} \egdef \bigwedge_{i \in \interval{1}{n}}\avarprop_i$, which reflects the encoding of $2^n-1$.

This concludes the definition of $\complete{1}$ (and $\completeplus{1}$), which is proven correct with respect to its specification.

\begin{lemma}
Let $\amodel,\aworld \models \init{1}$. We have $\amodel,\aworld \models \complete{1}$ iff $\pair{\amodel}{\aworld}$ satisfies \ref{prop:apS_1}, \ref{prop:apZ_1},
\ref{prop:apU_1}, \ref{prop:apC_1} and \ref{prop:apA}.
\end{lemma}

\paragraph{Inductive case: $1 \leq i < j$ and $j \geq 2$.}
We now define
\begin{nscenter}
\hfill $\fork{\aaux}{\aauxbis}{i}{j}$,
\hfill $\less{\aaux}{\aauxbis}{i}{j}$,
\hfill $\successor{\aaux}{\aauxbis}{j}$, \hfill\,\\
\hfill $\pU{j}$,
\hfill $\pC{j}$,
\hfill $\complete{j}$. \hfill\,
\end{nscenter}
where $1 \leq i < j$ and $j \geq 2$. As an implicit inductive hypothesis, used to prove that the formulae are well-defined, we assume that
$\successor{\aaux}{\aauxbis}{j'}$ and $\complete{j'}$ are already defined for every $j' < j$,
whereas $\fork{\aaux}{\aauxbis}{i'}{j'},$ and $\less{\aaux}{\aauxbis}{i'}{j'}$ are already defined for every $1 \leq i' \leq j'$ such that $j' - i' < j - i$.

According to its definition, as also depicted in Figure~\ref{figure-fork}, $\fork{\aaux}{\aauxbis}{i}{j}$ can be defined as follows:
\[
    \fork{\aaux}{\aauxbis}{i}{j} \egdef \fork{\aaux}{\aauxbis}{i}{i} \land \HMBox{\avartree}^i\completeplus{j-i}.
\]
It is easy to see that this formula is well-defined: $\fork{\aaux}{\aauxbis}{i}{i}$ is a formula of the base case, whereas $\completeplus{j {-} i}$ is defined by inductive hypothesis, since we have $j-i < j$.

Let us now consider the formula $\less{\aaux}{\aauxbis}{i}{j}$. Under the hypothesis that $\amodel,\aworld \models \fork{\aaux}{\aauxbis}{i}{j}$, we recall that this formula must check whether
 $\nb{\aworld_{\aaux}} < \nb{\aworld_{\aauxbis}}$ holds for the two (distinct) worlds $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation^i(\aworld)$ corresponding to the nominal $\aaux$ and $\aauxbis$, respectively.
 Since $i < j$, $\nb{\aworld_{\aaux}}$ and $\nb{\aworld_{\aauxbis}}$ are encoded using the truth value of $\treeval$ on the $\avartree$-children
 of $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$, respectively. In order to rely on the same arithmetical properties of binary numbers used to define $\less{\aaux}{\aauxbis}{j}{j}$ (base case),
we need to find two partitions
 $P_\aaux = \{L_\aaux,S_\aaux,R_\aaux\}$ and $P_\aauxbis = \{L_\aauxbis,S_\aauxbis,R_\aauxbis\}$ of the $\avartree$-children of $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$, respectively, such that:
 \begin{description}
   \item[\desclabel{(LSR)}{desc:LSR}:] Given $b \in \{\aaux,\aauxbis\}$, $P_b$ split the $\avartree$-children as follows:
 \begin{itemize}
   \item there is a $\avartree$-children $s_b$ of $\aworld_{b}$ such that $S_b = \{s_b\}$;
   \item $\nb{r} < \nb{s_b} < \nb{l}$, for every $r \in R_b$ and $l \in L_b$.
 \end{itemize}
 \item[\desclabel{(LESS)}{desc:LESS}:] $P_{\aaux}$ and $P_{\aauxbis}$ have the arithmetical properties of $<$ :
  \begin{itemize}
    \item $\nb{s_\aaux} = \nb{s_\aauxbis}$, $\amodel,s_\aaux \models \lnot \treeval$ and $\amodel,s_\aauxbis \models \treeval$;
    \item
      for every $l_\aaux \in L_\aaux$ and $l_\aauxbis \in L_\aauxbis$, if $\nb{l_\aaux} = \nb{l_\aauxbis}$
      then $\amodel,l_\aaux \models \treeval$ $\iff$ $\amodel,l_\aauxbis \models \treeval$.
  \end{itemize}
\end{description}
It is important to notice that these conditions essentially revolves around the numbers encoded by $\avartree$-children, which be compared using the already defined (by inductive reasoning) formulae $\less{\aaux}{\aauxbis}{i'}{j'}$, where $j'-i' < j - i$.
Since the semantics of $\less{\aaux}{\aauxbis}{i}{j}$ is given under the hypothesis that $\amodel,\aworld \models \fork{\aaux}{\aauxbis}{i}{j}$, we can assume that every children of $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$ has every $\Aux$-children.
Then, we rely on the auxiliary propositions $\{\avarleft, \avarselect, \avarright\}$ in order to mimic the reasoning done in~\ref{desc:LSR} and~\ref{desc:LESS}.

We start by considering the constraint involved in \ref{desc:LSR} and express them with the formula $\lsrpartition{j}$, which is satisfied by a pointed forest $\pair{\amodel = (\worlds,\arelation,\avaluation)}{\aworld}$ whenever:
\begin{itemize}
  \item $\pair{\amodel}{\aworld}$ satisfies $\complete{j}$;
  \item Every $\avartree$-child of $\aworld$ has exactly one $\{\avarleft,\avarselect,\avarright\}$-child, and
  only one of these $\avartree$-children (say $\aworld'$) has a $\avarselect$-child;
  \item Every $\avartree$-child of $\aworld$ that has an $\avarleft$-child encodes a number greater than $\nb{\aworld'}$;
  \item Every $\avartree$-child of $\aworld$ that has a $\avarright$-child encodes a number smaller than $\nb{\aworld'}$.
\end{itemize}
It should be noted that, despite this formula being defined in terms of $\complete{j}$, we only rely on $\lsrpartition{j-i}$ (which is defined by inductive reasoning) in order to define $\less{\aaux}{\aauxbis}{i}{j}$.
Figure~\ref{figure-lsr} schematise a model satisfying $\lsrpartition{j}$.
\begin{figure}
\begin{tikzpicture}
  \node (upleft) at (0,0) {};

  \path (upleft.center) -- ++(0.475\linewidth,-0.4) node[dot,label={$\aworld$}] (root) {.};

  \draw[pto] (root.center) -- ++ (-0.186\linewidth,-1.5) node[dot] (l1) {};
  \draw[pto] (root.center) -- ++ (-0.408\linewidth,-1.5) node[dot] (l2) {};
  \draw[pto] (root.center) -- ++ (0,-1.5) node[dot] (c1) {};
  \draw[pto] (root.center) -- ++ (0.186\linewidth,-1.5) node[dot] (r1) {};
  \draw[pto] (root.center) -- ++ (0.408\linewidth,-1.5) node[dot] (r2) {};

  \path (root.center) -- ++ (-0.2975\linewidth,-1.5) node (dots) {$\scaleobj{1.8}{\dots}$};
  \path (root.center) -- ++ (0.2975\linewidth,-1.5) node (dotsbis) {$\scaleobj{1.8}{\dots}$};


  \path (root.center) -- ++ (0.2975\linewidth,-2.2) node (min1) {$\scaleobj{1.3}{<}$};
  \path (root.center) -- ++ (0.09\linewidth,-2.2) node (min2) {$\scaleobj{1.3}{<}$};
  \path (root.center) -- ++ (-0.2975\linewidth,-2.2) node (min3) {$\scaleobj{1.3}{<}$};
  \path (root.center) -- ++ (-0.09\linewidth,-2.2) node (min4) {$\scaleobj{1.3}{<}$};

  \foreach \x in {l1,l2,c1,r1,r2} {
    \path (\x.center) -- ++ (-0.066\linewidth,-1.2) node (l\x) {};
    \path (\x.center) -- ++ (0.066\linewidth,-1.2) node (r\x) {};

      \draw[gray!30,fill=gray!30] (\x.center) -- (l\x.center) -- (r\x.center) -- (\x.center);
      \draw[alin] (\x.center) -- (l\x.center);
      \draw[alin] (\x.center) -- (r\x.center);
  }

  \path (upleft) -- ++(0.95\linewidth,0) node[label={[xshift=-42pt,yshift=-16pt]$\scaleobj{0.8}{\lsrpartition{j}, \text{ implies } \complete{j}}$}] (upright) {};
  \path let \p1 = (e1ll1) in (upleft) -- ++ (0,\y1) node (bottomleft) {};
  \path let \p1 = (e1ll1) in (upright) -- ++ (0,\y1) node (bottomright) {};

  \path (upleft) -- ++ (0,-1.7) node (midleft) {};
  \path (upright) -- ++ (0,-1.7) node (midright) {};

  \path (midleft) -- ++ (0.42\linewidth,0) node (selectleft) {};
  \path (midright) -- ++ (-0.42\linewidth,0) node (selectright) {};

  \path (midleft) -- ++ (0,-0.4) node (downleft) {};
  \path (midright) -- ++ (0,-0.4) node (downright) {};

  \path (downleft) -- ++ (0.42\linewidth,0) node (selectleftbottom) {};
  \path (downright) -- ++ (-0.42\linewidth,0) node (selectrightbottom) {};

  \begin{pgfonlayer}{bg0}

    \draw[gray!15,fill=gray!15] (selectright.center) -- (selectrightbottom.center) -- (downright.center) -- (midright.center) -- (selectright.center);


    \draw[gray!30,fill=gray!30] (selectleft.center) -- (selectleftbottom.center) -- (selectrightbottom.center) -- (selectright.center) -- (selectleft.center);


    \draw[gray!60,fill=gray!60] (selectleft.center) -- (selectleftbottom.center) -- (downleft.center) -- (midleft.center) -- (selectleft.center);

  \end{pgfonlayer}

  \draw[aux] (l1) -- ++(-0.32,0.32) node[label={[xshift=-3pt,yshift=-10pt]$\avarleft$}] (labl1) {};
  \draw[aux] (l2) -- ++(-0.32,0.32) node[label={[xshift=-3pt,yshift=-10pt]$\avarleft$}] (labl2) {};

  \draw[aux] (c1) -- ++(0.32,0.32) node[label={[xshift=3pt,yshift=-10pt]$\avarselect$}] (labc1) {};

  \draw[aux] (r1) -- ++(0.32,0.32) node[label={[xshift=3pt,yshift=-10pt]$\avarright$}] (labr1) {};
  \draw[aux] (r2) -- ++(0.32,0.32) node[label={[xshift=3pt,yshift=-10pt]$\avarright$}] (labr2) {};

\end{tikzpicture}
\caption{Shape of a model satisfying $\lsrpartition{j}$.}
\label{figure-lsr}
\end{figure}

\noindent The definition of $\lsrpartition{j}$ follows closely its specification:
\[
\begin{aligned}
\lsrpartition{j} \egdef \complete{j} \land \HMBox{\avartree}\Diamond_{=1}(\avarleft \lor \avarselect \lor \avarright)
\land \nominal{\avarselect}{1} \land\\
\lnot (\true \separate (\fork{\avarselect}{\avarleft}{1}{j} \land \lnot \less{\avarselect}{\avarleft}{1}{j})) \land\\
\lnot (\true \separate (\fork{\avarselect}{\avarright}{1}{j} \land \lnot \less{\avarright}{\avarselect}{1}{j})).
\end{aligned}
\]

We define the formula $\less{\aaux}{\aauxbis}{i}{j}$ as follows:
\[
  \true \separate \big(
    \twonoms{\aaux}{\aauxbis}{i} \land \HMBox{\avartree}^i\lsrpartition{j-i} \land
  \selectpred{\aaux}{\aauxbis}{i}{j} \land \leftpred{\aaux}{\aauxbis}{i}{j}
  \big)
\]
where $\selectpred{\aaux}{\aauxbis}{i}{j}$ and $\leftpred{\aaux}{\aauxbis}{i}{j}$ check the first and second condition in~\ref{desc:LESS}, respectively. In particular, by defining
$\equivalent{\aaux}{\aauxbis}{i}{j} \egdef \lnot (\less{\aaux}{\aauxbis}{i}{j} \lor \less{\aauxbis}{\aaux}{i}{j})$, we have
\[
\begin{aligned}
  & \selectpred{\aaux}{\aauxbis}{i}{j} \egdef
  \true \separate \big( \fork{\avariable}{\avariablebis}{i+1}{j} \land
  \atnom{\aaux}{i}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariable)\, \land\\
  &\pushright{\atnom{\aauxbis}{i}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariablebis) \land \equivalent{\avariable}{\avariablebis}{i+1}{j} \land \atnom{\avariable}{i+1}\lnot \treeval \land \atnom{\avariablebis}{i+1}\treeval
  \big);}\\
  &\leftpred{\aaux}{\aauxbis}{i}{j} \egdef \lnot \big( \true \separate \big(
   \fork{\avariable}{\avariablebis}{i+1}{j} \land
   \atnom{\aaux}{i}\HMDiamond{\avartree}(\Diamond \avarleft \land \Diamond \avariable)\, \land\\
  &\pushright{\ \, \atnom{\aauxbis}{i}\!\HMDiamond{\avartree}(\Diamond \avarleft \land \Diamond \avariablebis)
   \land  \equivalent{\avariable}{\avariablebis}{i+1}{j}{\land}
   \lnot (\atnom{\avariable}{i+1}\treeval \iff \atnom{\avariablebis}{i+1}\treeval)
  \big)\big).}
\end{aligned}
\]
Notice that both $\fork{\avariable}{\avariablebis}{i+1}{j}$ and $\equivalent{\avariable}{\avariablebis}{i+1}{j}$ used in these formulae are defined by inductive reasoning.
Let us briefly explain the formula $\selectpred{\aaux}{\aauxbis}{i}{j}$.
Suppose that $\pair{\amodel}{\aworld}$ satisfies $\twonoms{\aaux}{\aauxbis}{i} \land \HMBox{\avartree}^i\lsrpartition{j-i}$, as required by $\less{\aaux}{\aauxbis}{i}{j}$.
Let $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$ be the two worlds corresponding to the two nominals (at depth $i$) $\aaux$ and $\aauxbis$. Since
$\pair{\amodel}{\aworld} \models \HMBox{\avartree}^i\lsrpartition{j-i}$,
the $\avartree$-children of $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$ can be partitioned respectively in two sets
$P_\aaux = \{L_\aaux,\{s_\aaux\},R_\aaux\}$ and $P_\aauxbis = \{L_\aauxbis,\{s_\aauxbis\},R_\aauxbis\}$ satisfying \ref{desc:LSR}.
The formula $\selectpred{\aaux}{\aauxbis}{i}{j}$ states that there is a submodel $\amodel' \sqsubseteq \amodel$ such that
\begin{enumerate}[label=\Roman*.,align = left]
  \item $\amodel', \aworld \models \fork{\avariable}{\avariablebis}{i+1}{j}$;
  \item $s_\aaux$ corresponds to the nominal $\avariable$, at depth $i+1$;
  \item $s_\aauxbis$ corresponds to the nominal $\avariablebis$, at depth $i+1$;
  \item[IV-VI.] $\nb{s_\aaux} = \nb{s_\aauxbis}$, $\amodel,s_\aaux \not\models \treeval$ and $\amodel,s_\aauxbis \models \treeval$.
\end{enumerate}
(The enumeration I-VI refers to the conjuncts in the formula)

\noindent Thus, $\selectpred{\aaux}{\aauxbis}{i}{j}$ correctly models the first condition of~\ref{desc:LESS}.
Regarding $\leftpred{\aaux}{\aauxbis}{i}{j}$ and~\ref{desc:LESS}, a similar analysis can be performed.
in~. We define $\selectleftpred{\aaux}{\aauxbis}{i}{j}\egdef\leftpred{\aaux}{\aauxbis}{i}{j} \land \selectpred{\aaux}{\aauxbis}{i}{j}$.

Let us node consider the formula $\successor{\aaux}{\aauxbis}{j}$.
under the hypothesis that $\amodel,\aworld \models \fork{\aaux}{\aauxbis}{i}{j}$, this formula must check whether
 $\nb{\aworld_{\aauxbis}} = \nb{\aworld_{\aaux}} + 1$ holds for the two (distinct) worlds $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation^i(\aworld)$ corresponding to the nominal $\aaux$ and $\aauxbis$, respectively.
 Then, similarly to $\less{\aaux}{\aauxbis}{i}{j}$, according to the arithmetical properties of binary numbers we search for two partitions
 $P_\aaux = \{L_\aaux,S_\aaux,R_\aaux\}$ and $P_\aauxbis = \{L_\aauxbis,S_\aauxbis,R_\aauxbis\}$ of the $\avartree$-children of $\aworld_{\aaux}$ and $\aworld_{\aauxbis}$, respectively, such that $P_\aaux$ and $P_\aauxbis$ satisfy \ref{desc:LSR} and moreover
 \begin{description}
 \item[\desclabel{(PLUS)}{desc:PLUS}:] $P_{\aaux}$ and $P_{\aauxbis}$ have the arithmetical properties of $+1$ :
  \begin{itemize}
    \item $P_{\aaux}$ and $P_{\aauxbis}$ satisfy \ref{desc:LESS};
    \item
      for every $r_\aaux \in R_\aaux$ we have $\amodel,r_\aaux \models \treeval$;
    \item  for every $r_\aauxbis \in R_\aauxbis$ we have $\amodel,r_\aaux \not\models \treeval$.
  \end{itemize}
\end{description}
where $S_\aaux = \{s_\aaux\}$ and $S_{\aauxbis} = \{s_\aauxbis\}$, as required by \ref{desc:LSR}.

The definition of $\successor{\aaux}{\aauxbis}{j}$ is similar to $\less{\aaux}{\aauxbis}{i}{j}$:
\[
  \true  {\separate} \big(
    \twonoms{\aaux}{\aauxbis}{1} \land \HMBox{\avartree}\lsrpartition{j-1} \land
    \selectleftpred{\aaux}{\aauxbis}{1}{j}
    \land
    \rightpred{\aaux}{\aauxbis}
  \big)
\]
where $\rightpred{\aaux}{\aauxbis} \egdef \atnom{\aaux}{1}\HMBox{\avartree}(\Diamond \avarright \implies \treeval)
\land \atnom{\aauxbis}{1}\HMBox{\avartree}(\Diamond \avarright \implies \lnot \treeval) $
captures the last two conditions of~\ref{desc:PLUS}.

It remains to define the formulae $\pU{j}$ and $\pC{j}$, which essentially rely on the formulae $\fork{\aaux}{\aauxbis}{i}{j}$, $\less{\aaux}{\aauxbis}{i}{j}$ and $\successor{\aaux}{\aauxbis}{j}$.
The formula $\pU{j}$ is defined similarly to $\pU{1}$:
since a model satisfying $\complete{j}$ satisfies the formula $\pA$,
every $\avartree$-node in $\arelation(\aworld)$ has two auxiliary children, one $\avariable$-node and one $\avariablebis$-node. Then, for the formula $\pU{j}$ we can use these two children and rely on the $\separate$ operator to state that it is not possible to find a submodel of $\amodel$ such that $\aworld$ only has two distinct children $\aworld_{\avariable}$ and $\aworld_{\avariablebis}$ corresponding to the nominals $\avariable$ and $\avariablebis$ and
such that $\nb{\aworld_\avariable} = \nb{\aworld_\avariablebis}$.
\[
\pU{j} = \lnot \big(\true \separate (\fork{\avariable}{\avariablebis}{1}{j} \land \equivalent{\avariable}{\avariablebis}{1}{j})\big)
\]

The formula $\pC{j}$ is also very similar to $\pC{1}$:
\[
\begin{aligned}
\pC{j} \egdef &\lnot
  \Big( \Box \false \separate
    \Big(\HMBox{\avartree} (\completeplus{j-1} \land \Diamond \avariablebis) \land
    \nominal{\avariable}{1}
 \land \\
 & \atnom{\avariable}{1} \lnot \one_{j} \land \lnot \big( \true \separate (\fork{\avariable}{\avariablebis}{1}{j} \land
 \successor{\avariable}{\avariablebis}{j})\big)\Big)\Big)
\end{aligned}
\]
where $\one_j \egdef \HMBox{\avartree} \treeval$ reflects the encoding of $\amapter(j,n)-1$ for $j > 1$.
The main difference between $\pC{1}$ and $\pC{j}$ ($j > 1$) is that the conjunct $\HMBox{\avartree}\Diamond \avariablebis$ of $\pC{1}$ is replaced by $\HMBox{\avartree} (\completeplus{j-1} \land \Diamond \avariablebis)$
in $\pC{j}$, as needed to correctly evaluate $\fork{\avariable}{\avariablebis}{1}{j}$.
Indeed, the difference between $\fork{\avariable}{\avariablebis}{1}{1}$ and $\fork{\avariable}{\avariablebis}{1}{j}$ is precisely that the latter requires $\HMBox{\avartree}\completeplus{j-1}$.

The definition of $\complete{j}$ is now complete. We prove that it is correct with respect to its specification.

\begin{lemma}
Let $\amodel,\aworld \models \init{j}$. We have $\amodel,\aworld \models \complete{j}$ iff $\pair{\amodel}{\aworld}$ satisfies \ref{prop:apS}, \ref{prop:apZ},
\ref{prop:apU}, \ref{prop:apC} and \ref{prop:apA}.
\end{lemma}

The size of $\complete{j}$ is exponential in $j > 1$ and polynomial in $n \geq 1$.
As its size is therefore elementary, we can use this formula as a starting point to reduce $\tiling_k$.


==> sections/OLD-section-tiling-SC.tex <==
%!TEX root = ../main.tex

\subsection{Tiling a $\amapter(k,n) \times \amapter(k,n)$ grid.}
After the efforts needed in order to define the formula $\complete{j}$,
we are ready to  prove the \tower-hardness of
$\satproblem{\modallogicSC}$ with a uniform reduction from $\tiling_k$, for every $k \geq 2$.

Let $k \geq 2$ and let $\pair{\cTT}{\atile}$ be an instance of
$\tiling_k$, where $\cTT = \triple{\cT}{\cH}{\cV}$ and $\atile \in \cT$.
In the following, we define a formula $\atiling{k}{\cTT,\atile}$ such that the following lemma holds.

\begin{lemma}\label{lemma:tiling_correct_encoding}
$\pair{\cTT}{\atile}$ as a solution for $\tiling_k$ if and only if
the formula $\atiling{k}{\cTT,\atile}$ is satisfiable.
\end{lemma}

Recall that a solution for $\pair{\cTT}{\atile}$ w.r.t. $\tiling_k$ is a map
$\tau: \interval{0}{\amapter(k,n)-1} \times \interval{0}{\amapter(k,n)-1} \to \cT$
satisfying~\ref{tiling_c:1} and~\ref{tiling_c:2}.
W.l.o.g.\ we assume $\cT$ to be a set of atomic propositions, disjoint form the sets $\{\avarprop_1,\dots,\avarprop_n,\treeval\}$ and $\Aux$ used in the definition of $\complete{j}$.
Let us first describe how to to represent a $\interval{0}{\amapter(k,n)-1}^2$ grid in a pointed forest
$\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$.
We use the same ideas needed in order to define $\complete{k}$, but with some minor modifications.
As previously stated, if $\amodel,\aworld \models \complete{k}$ then
given a $\avartree$-node $\aworld' \in \arelation(\aworld)$,
the number $\nb{\aworld'} \in \interval{0}{\amapter(k,n)-1}$ is encoded using the $\avartree$-children of $\aworld'$, where the numbers encoded by these children represent positions
in the binary encoding of $\nb{\aworld'}$.
Instead of being a single number, a position in the grid is a pair of numbers  $(h,v) \in \interval{0}{\amapter(k,n)-1}^2$.
Hence, in a model $\pair{\amodel}{\aworld}$ satisfying $\atiling{k}{\cTT,\atile}$
we require that $\aworld' \in \arelation(\aworld)$ encodes two numbers $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$, and say that $\aworld'$ encodes the position $(h,v)$ if and only if $\nbexp{\aworld'}{\cH} = h$ and $\nbexp{\aworld'}{\cV} = v$.
Since both numbers are from $\interval{0}{\amapter(k,n)-1}$, we can use the same amount of $\avartree$-children as in $\complete{k}$ in order to encode both $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$.
Thus, we rely on the formula $\complete{k-1}$ in order to force $\aworld'$ to have the correct amount of $\avartree$-children, by requiring it to hold in $\pair{\amodel}{\aworld'}$.
Similarly to what we have done for $\complete{j}$ ($j \geq 2$) in the previous section, we encode the numbers $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$
by using the truth value, on the $\avartree$-children of $\aworld'$, of two new atomic propositions $\treeval_\cH$ and $\treeval_\cV$, respectively.
We then use similar formulae to $\pZ{k}$, $\pU{k}$ and $\pC{k}$ in order to state that $\aworld$ witness exactly one children for each position in the grid. Once the grid is encoded, the tiling conditions can be enforced rather easily.

We introduce the formula $\agrid{k}{\cTT}$ that characterise the set of models encoding the $\interval{0}{\amapter(k,n)-1}^2$ grid.
A model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying
$\agrid{k}{\cTT}$ is such that:
\begin{description}
  \item[\desclabel{(\apZ$_{\cTT,k}$)}{tiling_enc:apZ}] One $\avartree$-node in $\arelation(\aworld)$ encodes the position $\pair{0}{0}$, i.e. there is an $\avartree$-node $\tilde\aworld{\in}\,\arelation(\aworld)$ s.t.\
    $\nbexp{\tilde\aworld}{\cH} = \nbexp{\tilde\aworld}{\cV} = 0$;
  \item[\desclabel{(\apU$_{\cTT,k}$)}{tiling_enc:apU}] for every two distinct $\avartree$-nodes $\aworld_1,\aworld_2 \in \arelation(\aworld)$, $\nbexp{\aworld_1}{\cH} \neq \nbexp{\aworld_2}{\cH}$ or  $\nbexp{\aworld_1}{\cH} \neq \nbexp{\aworld_2}{\cH}$;
  \item[\desclabel{(\apC$_{\cTT,k}$)}{tiling_enc:apC}] for every $\avartree$-node $\aworld_1 \in \arelation(\aworld)$,
  \begin{itemize}
    \item if $\nbexp{\aworld_1}{\cH} < \amapter(j,n)-1$ then $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}+1$ and $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}$, for some $\avartree$-node $\aworld_2 \in \arelation(\aworld)$;
    \item if $\nbexp{\aworld_1}{\cV} < \amapter(j,n)-1$ then $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}+1$ and $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}$, for some $\avartree$-node $\aworld_2 \in \arelation(\aworld)$;
  \end{itemize}
  \item[\desclabel{(\ainit/\apS/\apA)}{tiling_enc:apS}] $\pair{\amodel}{\aworld}$ satisfies $\init{k}$,  $\pS{k}$ and $\pA$;
\end{description}
It is easy to see that, with these conditions, $\pair{\amodel}{\aworld}$ correctly encodes the grid.
The definition of $\agrid{k}{\cTT}$ follows rather closely the definition of $\complete{j}$.
It is defined as
\[
    \pZT{k}{\cTT} \land \pUT{k}{\cTT} \land \pCTBB{k}{\cTT} \land \init{k} \land \pS{k} \land \pA
\]
where each conjunct express the homonymous property above.
In order to define the first three conjuncts of $\agrid{k}{\cTT}$  (hence completing its definition)
we start by defining the formulae $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ and $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$, where $\heapdim \in \{\cH,\cV\}$. Similarly to $\equivalent{\aaux}{\aauxbis}{1}{k}$ and $\successor{\aaux}{\aauxbis}{k}$,
Given a model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying $\fork{\aaux}{\aauxbis}{1}{k}$, and the two $\avartree$-nodes $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation(\aworld)$
corresponding to the nominals $\aaux$ and $\aauxbis$, respectively,
\begin{itemize}
\item $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ states that $\nbexp{\aworld_{\aaux}}{\heapdim} = \nbexp{\aworld_{\aauxbis}}{\heapdim}$;
\item $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ states that $\nbexp{\aworld_{\aauxbis}}{\heapdim} = \nbexp{\aworld_{\aaux}}{\heapdim}+1$.
\end{itemize}
To encode $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ we simply require that for every two $\avartree$-children $\aworld_{\avariable} \in \arelation(\aworld_{\aaux})$ and $\aworld_{\avariablebis} \in \arelation(\aworld_{\aauxbis})$, if
$\nb{\aworld_{\avariable}} = \nb{\aworld_{\avariablebis}}$ then $\aworld_{\avariable}$ and $\aworld_{\avariablebis}$
agree on the satisfaction of $\treeval_\heapdim$. In formula:
\[
\begin{aligned}
  \bequivalent{\aaux}{\aauxbis}{k}{\heapdim}
  \egdef
  \lnot \big( \true \separate & (\fork{\avariable}{\avariablebis}{2}{k}
  \land \atnom{\aaux}{1}{\HMDiamond{\avartree} \Diamond \avariable}
  \land \atnom{\aauxbis}{1}{\HMDiamond{\avartree} \Diamond \avariablebis}
  \\ & \land \equivalent{\avariable}{\avariablebis}{2}{k}
  \land \lnot (\atnom{\avariable}{2}\treeval_\heapdim \iff \atnom{\avariablebis}{2}\treeval_\heapdim)
  )\big).
\end{aligned}
\]
The formula $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ can be defined by slightly modifying the formula $\successor{\aaux}{\aauxbis}{k}$. We start by defining the formulae $\bleftpred{\aaux}{\aauxbis}{k}{\heapdim}$, $\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}$ and $\brightpred{\aaux}{\aauxbis}{\heapdim}$
with semantics similar to $\leftpred{\aaux}{\aauxbis}{1}{k}$, $\selectpred{\aaux}{\aauxbis}{1}{k}$
and $\rightpred{\aaux}{\aauxbis}$, respectively, but where, for a given $\avartree$-node in $\arelation^2(\aworld)$,
we are interested in the satisfaction of $\treeval_\heapdim$ instead of $\treeval$. For example, the formula $\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}$ is defined as
\[
\begin{aligned}
  & \bselectpred{\aaux}{\aauxbis}{k}{\heapdim}\egdef
  \true \separate \big( \fork{\avariable}{\avariablebis}{2}{k} \land
  \atnom{\aaux}{1}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariable)\, \land\\
  &\ \ \atnom{\aauxbis}{1}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariablebis) \land \equivalent{\avariable}{\avariablebis}{2}{k} \land \atnom{\avariable}{2}\lnot \treeval_\heapdim \land \atnom{\avariablebis}{2}\treeval_\heapdim
  \big)
\end{aligned}
\]
i.e. by replacing the two last conjuncts of $\selectpred{\aaux}{\aauxbis}{1}{k}$, $\atnom{\avariable}{2}\lnot \treeval $ and $\atnom{\avariablebis}{2}\treeval$ with $\atnom{\avariable}{2}\lnot \treeval_\heapdim$ and $\atnom{\avariablebis}{2}\treeval_\heapdim$, respectively.
Similarly, $\bleftpred{\aaux}{\aauxbis}{k}{\heapdim}$ is defined from $\leftpred{\aaux}{\aauxbis}{1}{k}$ by replacing the last conjunct of this formula, i.e.\ $\lnot (\atnom{\avariable}{2}\treeval \iff \atnom{\avariablebis}{2}\treeval)$, by
$\lnot (\atnom{\avariable}{2}\treeval_\heapdim \iff \atnom{\avariablebis}{2}\treeval_\heapdim)$.
Lastly, $\brightpred{\aaux}{\aauxbis}{\heapdim}$ is defined from $\rightpred{\aaux}{\aauxbis}$ by replacing every occurrence of $\treeval$ by $\treeval_\heapdim$.
The formula $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ is then defined as follows:
\[
\begin{aligned}
\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim} & \egdef
\true \separate
  \big(
     \twonoms{\aaux}{\aauxbis}{1} \land \HMBox{\avartree}\lsrpartition{k-1} \land\\
    & \ \, \bleftpred{\aaux}{\aauxbis}{k}{\heapdim}\,{\land}\,\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}\,{\land}\,
      \brightpred{\aaux}{\aauxbis}{\heapdim}
  \big).
\end{aligned}
\]
We are now ready to define the formulae $\pZT{k}{\cTT}$, $\pUT{k}{\cTT}$ and $\pCTBB{k}{\cTT}$, achieving the conditions \ref{tiling_enc:apZ}, \ref{tiling_enc:apU} and \ref{tiling_enc:apC}, respectively.
All these formulae follows closely the definitions of $\pZ{k}$, $\pU{k}$ and $\pC{k}$ of the previous sections, hence we refer to these latter formulae for an informal description on how they works. The formula $\pZT{k}{\cTT}$ is simply defined as $\HMDiamond{\avartree}(\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV))$.
The formula $\pUT{k}{\cTT}$ is defined from $\pZ{k}$ by simply replacing $\equivalent{\avariable}{\avariablebis}{1}{k}$
with $\bequivalent{\aaux}{\aauxbis}{k}{\cH} \land \bequivalent{\aaux}{\aauxbis}{k}{\cV}$:
\[
\pUT{k}{\cTT} = \lnot \big(\true \separate (\fork{\avariable}{\avariablebis}{1}{k} \land \bequivalent{\avariable}{\avariablebis}{k}{\cH} \land\bequivalent{\avariable}{\avariablebis}{k}{\cV})\big)
\]
Lastly, $\pCTBB{k}{\cTT} \egdef \pCTB{k}{\cTT}{\cH} \land \pCTB{k}{\cTT}{\cV}$ where
\[
\begin{aligned}
&\pCTB{k}{\cTT}{\cH} \egdef \lnot
  \Big( \Box \false\!\separate\!
    \Big(\HMBox{\avartree} (\completeplus{k{-}1}\,{\land}\,\Diamond \avariablebis)\,{\land}\,
    \nominal{\avariable}{1} \\
 &\ \land
 \atnom{\avariable}{1} \lnot \one^{\cH}_{k} \land \lnot \big( \true \separate (\fork{\avariable}{\avariablebis}{1}{j} \land
 \bsuccessor{\avariable}{\avariablebis}{k}{\cH}
 \land \bequivalent{\avariable}{\avariablebis}{k}{\cV}
 )\big)\Big)\Big)
\end{aligned}
\]
and $\pCTB{k}{\cTT}{\cV}$ is defined form $\pCTB{k}{\cTT}{\cH}$ by replacing $\one^{\cH}_{k}$, $\bsuccessor{\avariable}{\avariablebis}{k}{\cH}$ and
$\bequivalent{\avariable}{\avariablebis}{k}{\cV}$ with
$\one^{\cV}_{k}$, $\bsuccessor{\avariable}{\avariablebis}{k}{\cV}$ and
$\bequivalent{\avariable}{\avariablebis}{k}{\cH}$, respectively.
Here, $\one^{\heapdim}_{k}$ ($\heapdim \in \{\cH,\cV\}$) is defined as $\HMBox{\avartree} \treeval_\heapdim$,
and hence it is satisfied by the $\avartree$-nodes $\aworld' \in \arelation(\aworld)$ such that $\nbexp{\aworld'}{\heapdim} = \amapter(k,n)-1$.
This concludes the definition of $\agrid{k}{\cTT}$. It is proved correct in the following lemma.

\begin{lemma}
$\amodel,\aworld \models \agrid{k}{\cTT}$ if and only if $\pair{\amodel}{\aworld}$ satisfies \ref{tiling_enc:apZ}, \ref{tiling_enc:apU},
\ref{tiling_enc:apC} and \ref{tiling_enc:apS}.
\end{lemma}

We can now proceed to the encoding of the tiling conditions~\ref{tiling_c:1} and~\ref{tiling_c:2}.
Given a model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying
$\agrid{k}{\cTT}$, the existence of a solution for $\pair{\cTT}{\atile}$, w.r.t.\ $\tiling_k$, can be expressed with the following conditions:
\begin{description}
  \item[\desclabel{(\apone$_{\cTT}$)}{tiling_enc:one_tile}] every $\avarprop$-node in $\arelation(\aworld)$ satisfies exactly one tile in $\cT$;
  \item[\desclabel{(\apfirst$_{\cTT,\atile}$)}{tiling_enc:zero_c}] for $\tilde\aworld{\in}\,\arelation(\aworld)$, if $\nbexp{\tilde\aworld}{\cH} {=} \nbexp{\tilde\aworld}{\cV} {=} 0$ then $\tilde{\aworld} \in \avaluation(\atile)$;
  \item [\desclabel{(\aphor$_{\cTT}$)}{tiling_enc:hori}] for every $\aworld_1,\aworld_2 \in \arelation(\aworld)$,
    if $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}+1$ and $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}$ then there is $\pair{\atile_1}{\atile_2} \in \cH$ such that
    $\aworld_1 \in \avaluation(\atile_1)$ and $\aworld_2 \in \avaluation(\atile_2)$;
  \item [\desclabel{(\apvert$_{\cTT}$)}{tiling_enc:hori}] for every $\aworld_1,\aworld_2 \in \arelation(\aworld)$,
    if $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}+1$ and $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}$ then there is $\pair{\atile_1}{\atile_2} \in \cV$ such that
    $\aworld_1 \in \avaluation(\atile_1)$ and $\aworld_2 \in \avaluation(\atile_2)$.
\end{description}
Then, the formula $\atiling{k}{\cTT,\atile}$ can be defined as
\[
\agrid{k}{\cTT} \land \pone{\cTT} \land \pfirst{k}{\cTT,\atile} \land \phor{k}{\cTT} \land \pvert{k}{\cTT}
\]
where the last four conjuncts express the homonymous property above.
Given the toolkit of formulae introduced up to now, these four formulae are easy to define.
$\pone{\cTT}$ is simply defined as
$\HMBox{\avartree}\bigvee_{\atile_1 \in \cT} (\atile_1 \land \bigwedge_{\atile_2 \in \cT} \lnot \atile_2)$.
The formula $\pfirst{k}{\cTT,\atile}$ can be defined as
\[
\pfirst{k}{\cTT,\atile} \egdef \HMBox{\avartree}\big(\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV) \implies \atile\big)
\]
where we use the fact that
the $\avartree$-node $\aworld' \in \arelation(\aworld)$ encoding $\pair{0}{0}$ is the only one, among the $\avartree$-children of $\aworld$, satisfying $\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV)$.
For the formula $\phor{k}{\cTT}$, we essentially state that there cannot be two $\avartree$-nodes $\aworld_1,\aworld_2 \in \arelation(\aworld)$ such that $\aworld_2$ encodes the position $\pair{\nbexp{\aworld_1}{\cH}+1}{\nbexp{\aworld_1}{\cV}}$
and $\aworld_1 \in \avaluation(\atile_1)$, $\aworld_2 \in \avaluation(\atile_2)$ does not hold for any $\pair{\atile_1}{\atile_2} \in \cH$. In formula:
\[
\begin{aligned}
\phor{k}{\cTT} \egdef \lnot
\big(
\true
  \separate
  \big(&
  \fork{\avariable}{\avariablebis}{1}{k} \land
  \bsuccessor{\avariable}{\avariablebis}{k}{\cH}
  \land \bequivalent{\avariable}{\avariablebis}{k}{\cV}
  \\
  & \land
  \lnot \textstyle\bigvee_{{\pair{\atile_1}{\atile_2} \in \cH}} (\atnom{\avariable}{1} \atile_1 \land \atnom{\avariablebis}{1} \atile_2)
  \big)
\big).
\end{aligned}
\]
Lastly, $\pvert{k}{\cTT}$ is defined as $\phor{k}{\cTT}$, but replacing $\cH$ by $\cV$ and vice-versa
(in particular, in $\pvert{k}{\cTT}$ the last disjunction appearing in $\phor{k}{\cTT}$ becomes indexed by elements in $\cV$).
This conclude the definition of $\atiling{k}{\cTT,\atile}$, for which we show Lemma~\ref{lemma:tiling_correct_encoding}. We then derive the following result.

\begin{theorem}
  $\satproblem{\modallogicSC}$ is \tower-complete.
\end{theorem}


==> sections/OLD-section-tower-completeness-SC.tex <==
%!TEX root = ../main.tex

In this section, we show that the satisfiability problem for \modallogicSC is \tower-complete, i.e. complete for the class of all
problems of time complexity bounded by a tower of exponential whose height is an elementary function~\cite{Schmitz16}.
Given two integers $k,n \geq 0$, we inductively define the tetration function $\amapter$ as $\amapter(0,n) \egdef n$ and
$\amapter(k+1,n) = 2^{\amapter(k,n)}$. Intuitively, $\amapter(k,n)$ defines a tower of exponentials of height $k$.
By $k$-\nexptime we denote the class of all problems decidable with a nondeterministic Turing machine of working time
$\bigO(\amapter(k,p(n)))$ for some polynomial $p(.)$, on each input of length $n$.
In order to show \tower-hardness, it is then sufficient to show that there is a uniform elementary reduction that allows to prove
$k$-\nexptime-hardness for all $k$ greater than a certain (fixed) integer.
In our case, we achieve an exponential-space reduction from the $k$-\nexptime variant of the tiling problem (defined below), for every $k \geq 2$.

The tiling  problem $\tiling_k$ takes as input a triple $\cTT = \triple{\cT}{\cH}{\cV}$ where
$\cT$ is a finite set of tile types,
$\cH \subseteq \cT \times \cT$ (resp. $\cV \subseteq \cT \times \cT$) represents the horizontal
(resp. vertical) matching relation,
and an initial tile type $\atile \in \cT$.
A solution for the instance $\pair{\cTT}{c}$
is a mapping $\tau: \interval{0}{\amapter(k,n)-1} \times \interval{0}{\amapter(k,n)-1} \to \cT$ such that
\begin{description}
\itemsep 0 cm
\item[\desclabel{(first)}{tiling_c:1}] $\tau(0,0) = \atile$, and
\item[\desclabel{(hor\&vert)}{tiling_c:2}] for all $i\in \interval{0}{\amapter(k,n)-1}$ and $j \in \interval{0}{\amapter(k,n)-2}$, $\pair{\tau(j,i)}{\tau(j+1,i)} \in \cH\ $ and $\ \pair{\tau(i,j)}{\tau(i,j+1)} \in \cV$.
\end{description}
The problem of checking whether an instance of $\tiling_k$ has a solution is known to be $k$-\nexptime-complete (see \cite{CC-Papadimitriou}).

The reduction below from $\tiling_k$ to \satproblem{\modallogicSC}
recycles some ideas from~\cite{Bednarczyk&Demri19}
to reduce  $\tiling_k$ to the satisfiability problem for the second-order modal logic K over finite trees (let us call it MSOK(Trees))
Actually, in~\cite{Bednarczyk&Demri19} the presentation uses mainly quantified \CTL over trees restricted
to the next-time modality $\mathsf{EX}$.
In order to provide the adequate adaptation for \modallogicSC, we need to solve two major problems.
Firstly,  MSOK(Trees)
%% \QCTL
provides second-order quantification, whereas in \modallogicSC the second-order features are limited to the separating conjunction
$\separate$.
Secondly, the second-order quantification of
%% \QCTL
MSOK(Trees)
essentially colours the nodes in the tree-like Kripke structure while leaving the accessibility relation untouched.
The  operator $\separate$ in \modallogicSC modifies the accessibility relation, possibly making worlds that were reachable from the current world completely unreachable in submodels.
The \tower-hardness proof for \modallogicSC becomes then much more challenging: we would like to characterise the position on the grid encoded
by a world $\aworld$ by exploiting some properties of its descendants (similarly to what is done for
%% \QCTL),
MSOK(Trees)),
but at the same time we need to be careful and only consider submodels where $\aworld$ keeps encoding the same position.
In this sense, our encoding is robust: when the  operator $\separate$ is used to reason on submodels, we can enforce that no world
changes the position of the grid that it encodes.

\input{sections/section-nonelementary-children-SC}

\input{sections/section-tiling-SC}


==> sections/section-introduction.tex <==
%!TEX root = ../main.tex

\paragraph*{Logics with second-order features on trees.}
%% \paragraph{Logics with second-order features on trees.}
Arguably, trees are fundamental structures in computer science,  for instance
they correspond to the underlying structure behind many well-known
objects with a hierarchical topology. Moreover, tree representations are
desirable due to their good computational properties, such as the existence of
efficient search algorithms, and also the ability to \emph{dynamically change} (i.e., by adding nodes or by reason about submodels) without altering these good properties. Thus, it is natural to investigate languages
to formally reason about trees.

In the literature, there exists  a wide spectrum of languages designed to express and infer
properties about trees. For instance, many first-order dialects have been studied
looking for good computational properties (see e.g.~\cite{Benaimetal13,Bednarczyk&Charatonik&Kieronski17}). By contrast,
monadic second-order logic (\MSO)~\cite{Rabin69} occupies a special place due to the celebrated Rabin's theorem about
its decidability. However, the \tower-completeness\footnote{See the formal definition of \tower in~\cite{Schmitz16}.}
of its satisfiability problem
prevents us  from using systematically decision procedures dedicated to \MSO in order to solve (simple) reasoning tasks on trees.
As a consequence, other formalisms
raised, aiming for good computational behaviour but without
scarifying the  expressivity, as  provided, for example, by second-order quantification. In these languages, different aspects of the tree topology are
considered, i.e., some of them incorporate operations to talk about labelling,
while others may consider the accessibility relation.
%% SD 05/01/20 -- lack of space
%%  whereas others mix both kind
%% of properties.
Logics with propositional quantification~\cite{Fine70,Laroussinie&Markey14,Bednarczyk&Demri19}
introduce a way to reason about the possible labellings in the tree.
On the other hand, reachability predicates~\cite{Yorshetal05,Afanasievetal05,DemriLM18}
or more generally fixed-point operators~\cite{Bradfield&Walukiewicz18,Gheerbrant10}
allow us to explore nodes in a tree. Moreover, more specific
features have been included, sometimes leading to more specialised formalisms.
Among them, it is worth mentioning the use of arithmetical
constraints~\cite{Seidletal04,DalZilio&Lugiez06},
refinements essentially based on simulations~\cite{Bozzelli&vanDitmarsch&Pinchinat15}, or tree updates as in
context logic~\cite{CGZ05,Zarfaty07}.

In this article, we focus on the ability of reason about {\em submodels}
%% SD 05/01/20 use \defstyle when the term is defined, otherwise \em is fine.
to analyse trees in a structured way.
%%
%% SD 05/01/20 -- lack of space
%% This feature is the ability of reason
%% about \defstyle{submodels}.
%% This is a feature shared with at least
%% two particularly interesting families of logics.
%%
On the one hand, we consider composition operator as in ambient logics or
graph logics (see also~\cite{CCG03,CGZ05,Boneva&Talbot&Tison05,Dawar&Gardner&Ghelli07}), which decomposes
a tree into two disjoint pieces such that
once a node has been assigned to one submodel, all its descendants belong to the same submodel. On the other hand,
the separating conjunction from separation logic~\cite{Ishtiaq&OHearn01,OHearn&Reynolds&Yang01,Reynolds02,Demri&Fervari18} decomposes
the model
into two disjoint arbitrary submodels.
Obviously, these two operators are closely related
but
no uniform framework  investigates their relationships
%% between the induced specification languages,
regarding both their relative expressive power and computational complexity.
%%
%%
% This is certainly not an exhaustive list
% and, in the context of the current paper, it is worth also mentioning
% arithmetical
% constraints~\cite{Seidletal04,DalZilio&Lugiez06,Demri&Lugiez10},
% refinements essentially based on simulations~\cite{Bozzelli&vanDitmarsch&Pinchinat15}, or
% tree updates from context logic~\cite{CGZ05,Zarfaty07}.
% The wealth of languages is also naturally complemented by a wealth of tree-like structures considered
% in the logical formalisms, including labelled computation trees for temporal logics, finite labelled
% trees for ambient logics, graph logics or spatial logics~\cite{CCG03,CGZ05,Boneva&Talbot&Tison05,Dawar&Gardner&Ghelli07},
% data trees~\cite{Bojanczyketal09}, resource trees~\cite{Biri&Galmiche07}, feature trees~\cite{Jeannerod&Treinen18},
% or memory states for separation logics~\cite{Ishtiaq&OHearn01,OHearn&Reynolds&Yang01,Reynolds02}.
%%
\paragraph*{Our motivations.}
%% \paragraph{Our motivations.}
The wealth of languages is also naturally complemented by a wealth of tree-like structures considered
in the logical formalisms, including labelled computation trees for temporal
%% logics~\cite{Demri&Goranko&Lange16},
 logics,
finite labelled
trees for ambient logics, graph logics or spatial logics~\cite{CCG03,CGZ05,Boneva&Talbot&Tison05,Dawar&Gardner&Ghelli07},
%% SD 05/01/20 -- lack of space
%% data trees~\cite{Bojanczyketal09}, resource trees~\cite{Biri&Galmiche07}, feature trees~\cite{Jeannerod&Treinen18},
data trees~\cite{Figueira18},
or memory states for separation logics~\cite{Ishtiaq&OHearn01,OHearn&Reynolds&Yang01,Reynolds02}. Thus, the first step towards understanding
the effects of the aforementioned composition operators, is to pick  ``the right''
semantics. That is why,
%%
%% SD 05.01.20 -- lack of space
%%
%% we consider a semantics based on Kripke models
%% as in modal logics~\cite{Segerberg71,Blackburn&deRijke&Venema01}.
%% More precisely,
we interpret formulae on Kripke-style structures made of finite forests. This gives us a unifying and
standard semantics, while enabling us to take advantage of the  classical tools from modal logic~\cite{Blackburn&deRijke&Venema01}.

Thus, we are ready to focus on our main motivation: to investigate
the computational properties of logical formalisms with
operators to chop a
 tree.
%% , in particular, what are the properties of the resulting logics.
These logics do not appear out of the blue as this corresponds to
%%  are not arbitrary choices,
%% but they are
instances of the logic of bunched implications BI~\cite{Pym02,GalmicheBI}.
%%
%% SD 05.01.20 -- lack of space
%% So,
%%  from an abstract point of view,
%%  we deal with specific classes of {\em partial resource semigroups}.
%%
The benefits of this approach are twofold. First, we provide
 a uniform treatment of operations with the ability of splitting a tree into
disjoint pieces. In this way, we can come upon different behaviours in the BI
 family of logics. Secondly, as a by-product, we would like  to establish connections with other
logics introduced in the literature, and answer some open questions.
%% SD 27/12/19 --
%%  Therefore, our work is not merely a theoretical challenge.
%%
 For instance, it would allow us to study the relative expressivity between both chop operators
and the graded modal logic \GML~\cite{DeRijke00} or
to pinpoint the exact complexity  of the intensional
 fragment of static ambient logic without name restrictions $\SAL$~\cite{CCG03}.
%% SD 02/01/2020 Details are provided in the next paragraph.
\cut{
Furthermore, our modal logic approach allows us to
 make connections with the recently introduced modal separation logic with inverse modality ($\MSLminus$)
from~\cite{Demri&Fervari18}, and second-order modal logic on finite trees (herein called \msokt) from~\cite{Bednarczyk&Demri19}.
Finally, we are able
 to show the exact complexity bounds of the intensional
 fragment of static ambient logic without name restrictions $\SAL$~\cite{CCG03}, whose complexity was open for many years.
%%
% \begin{itemize}
%     % \item We introduce a uniform general framework to investigate logics for reasoning about composition of tree-like structures.
%     % \item We compare the different kinds of decomposing a tree. These choices come from the literature (e.g. ambient logic, separation logic), but their semantics are very different.
%     \item We provide a more standard semantic based on Kripke models, which allows us to use the modal logic tools.
%     \item An interesting point is that the more expressive logic is the one with lower complexity.
%     \item Establish some brief connection with \GML. Put an example of a complex formula in \GML that is simpler with $\modallogicCC$?
%     \item Maybe move the figures of \Cref{section-preliminaries} here?
%     \item Discuss connections with other logics: team logic~\cite{HannulaKVV18}, static ambient logic~\cite{CCG03,CGZ05}, (modal) separation logics, graph logics restricted to trees~\cite{Dawar&Gardner&Ghelli07}, one-agent refinement modal logic~\cite{Bozzelli&vanDitmarsch&Pinchinat15}, context logic, \cite{Zarfaty07}, spatial logics for trees~\cite{Boneva&Talbot&Tison05}, BI-loc~\cite{Biri&Galmiche07}.
% \end{itemize}
%% SD 17/10/2019
%% Revised version of "contributions" paragraph from CONCUR.
}
%% 
\paragraph*{Our contributions.}
%% \paragraph{Our contributions.}
We introduce the logics \modallogicCC and \modallogicSC interpreted on Kripke-style forest models,
equipped with the standard modality $\Diamond$, and respectively with the 
composition operator~$\chopop$ from static ambient logic~\cite{CCG03} and with
the separating conjunction~$\separate$ from separation logic~\cite{Ishtiaq&OHearn01,OHearn&Reynolds&Yang01,Reynolds02}. 
Both logical formalisms allow to state non-trivial properties about submodels but the binary modalities
$\chopop$ and $\separate$ operate differently: whereas~$\separate$
is able to decompose the models at any depth, $\chopop$ is much less permissive as the decomposition
is completely determined by what happens at the level of the children of the current node. 
Our contributions consist of a thorough comparison between  \modallogicCC and \modallogicSC
as far as expressivity and computational complexity are concerned. 
We show that \modallogicCC is as expressive as the graded modal logic~\GML~\cite{FattorosiBarnaba&DeCaro85,Tobies00}
whereas \modallogicSC is strictly less expressive than \GML. For instance, to show that 
\GML is strictly more expressive than~\modallogicSC,
we define  Ehrenfeucht-Fra\"iss\'e games for~\modallogicSC.
In terms of complexity, the satisfiability problem for~\modallogicCC is shown~\aexppol-complete\footnote{
\aexppol is the class of problems decidable by an alternating Turing machine working
in exponential-time and using only polynomially many alternations~\cite{Bozzelli17}.
It stands between~\nexptime and~\expspace.}.
The~\aexppol upper bound
amounts to establish an ex\-po\-nen\-tial-size model property, whereas the lower bound is by reducing
a satisfiability problem for an \aexppol-complete team logic~\cite{HannulaKVV18}.
Much more surprising,
we show that the satisfiability problem for~\modallogicSC  is \tower-complete.
The upper bound is a consequence of~\cite{Rabin69}
whereas \tower-hardness is shown by reduction from a \tower-complete tiling problem,
adapting substantially the \tower-hardness proof from~\cite{Bednarczyk&Demri19}.
In Section~\ref{section-other-logics}, we get the best of our results on 
\modallogicCC and \modallogicSC to solve several open problems. 
%% we present interesting by-products of our main results.
We relate~\modallogicCC
with an intensional fragment of static ambient logic~\SAL from~\cite{CCG03} by providing
polynomial-time reductions between their satisfiability problems. Consequently, we
establish~\aexppol-completeness of~\SAL, and goes against what
has been hinted in~\cite[Section 6]{CCG03}. Similarly, we establish that
the modal separation logic MSL($\Diamond^{-1},\separate$) from~\cite{Demri&Fervari18}
is \tower-complete.

%% SD 08/01/20 -- preparing the new introduction
\cut{
We introduce the modal logic~\modallogicCC  equipped with the modality~$\Diamond$
and the composition operator~$\chopop$ from static ambient logic~\cite{CCG03},
but interpreted on finite forests. Whereas it is rather obvious that~\modallogicCC is at least as expressive
as  graded modal logic~\GML, we establish that actually,~\modallogicCC is equally expressive with~\GML,
which is quite surprising in view of the second-order nature of $\chopop$.
We introduce its companion logic~\modallogicSC  equipped with the modality $\Diamond$
and the separating conjunction~$\separate$ from separation logic~\cite{Ishtiaq&OHearn01,OHearn&Reynolds&Yang01,Reynolds02}, again
interpreted on  finite forests. Unlike~$\chopop$, the separating conjunction~$\separate$
is able to separate the model at any depth of the trees. Whereas we show that~\modallogicSC
is not more expressive than~\GML, using developments about graded bisimulation from~\cite{DeRijke00}
and results for~\modallogicCC, we prove that~\GML is strictly more expressive than~\modallogicSC. In order to do that,
we define  Ehrenfeucht-Fra\"iss\'e games for~\modallogicSC.
These expressivity results are completed by characterising the computational complexity
of the satisfiability problem for~\modallogicCC, shown~\aexppol-complete\footnote{
\aexppol is the class of problems decidable by an alternating Turing machine working
in exponential-time and using only polynomially many alternations~\cite{Bozzelli17}.
It stands between~\nexptime and~\expspace.}.
The~\aexppol upper bound
amounts to establish an ex\-po\-nen\-tial-size model property, whereas the lower bound is by reducing
a satisfiability problem for an \aexppol-complete team logic~\cite{HannulaKVV18}.
Though~\modallogicSC is established strictly less expressive than~\modallogicCC,
we show that the satisfiability problem for~\modallogicSC  is \tower-complete.
The upper bound can be shown by a simple reduction into
the weak monadic second-order theory of one unary function shown decidable in~\cite{Rabin69}
whereas \tower-hardness is shown by reduction from a \tower-complete tiling problem,
adapting substantially the \tower-hardness proof from~\cite{Bednarczyk&Demri19}.
In Section~\ref{section-other-logics},
%% we present interesting by-products of our main results.
we relate~\modallogicCC
with an intensional fragment of static ambient logic~\SAL from~\cite{CCG03} by providing
polynomial-time reductions between their satisfiability problems. Consequently, we
establish~\aexppol-completeness of~\SAL, which solves an open problem and goes against what
has been hinted in~\cite[Section 6]{CCG03}. Similarly, we establish that
the modal separation logic MSL($\Diamond^{-1},\separate$) from~\cite{Demri&Fervari18}
is \tower-complete.
}

\noindent {\em Omitted proofs can be found in the technical appendix.}%%


==> sections/section-tiling-SC-short.tex <==
%!TEX root = ../main.tex
\subsection{Tiling a grid  $\interval{0}{\amapter(k,n)-1}  \times \interval{0}{\amapter(k,n)-1}$}\label{subsection:tiling-grid}
Now we are ready to prove the \tower-hardness of
$\satproblem{\modallogicSC}$ with a uniform reduction from $\tiling_k$, for every $k \geq 2$.

Let $k \geq 2$ and let $\pair{\cTT}{\atile}$ be an instance of
$\tiling_k$, where $\cTT = \triple{\cT}{\cH}{\cV}$ and $\atile \in \cT$.
In the following, we define a formula $\atiling{k}{\cTT,\atile}$ such that the following lemma holds.

\begin{lemma}\label{lemma:tiling_correct_encoding}
$\pair{\cTT}{\atile}$ as a solution for $\tiling_k$ if and only if
the formula $\atiling{k}{\cTT,\atile}$ is satisfiable.
\end{lemma}

Recall that for encoding a position of a grid, we need a pair of two numbers 
$(h,v) \in \interval{0}{\amapter(k,n)-1}^2$ representing the horizontal 
and the vertical positions. We already introduced how to encode numbers in 
binary representation in \Cref{subsec:nonelemchildren}.  
Since $(h,v) \in \interval{0}{\amapter(k,n)-1}^2$, for encoding each
position $(h,v)$, a world needs the same amount of children as for $\complete{k}$. 
This property allows us to characterise the set of models
$(\amodel=\tup{\worlds,\arelation,\avaluation},\aworld)$ 
encoding the grid  $\interval{0}{\amapter(k,n)-1}^2$. 
First, we need to establish that the grid has the intended shape.
For instance, we need to express that there is a node 
encoding position $(0,0)$, and also the grid contains all the required positions (e.g. for a node encoding a position $(i,j)$ with $j<\amapter(j,n)-1$, there exists a node encoding position $(i,j+1)$).
Notice that these conditions rely on the definition of properties as 
those introduced for $\complete{k}$, such as the relations `$<$' and `$+1$',
or the predicates $\pC{j}$, $\init{j}$ and $\pA$. In the same way, we can define the tiling conditions~\ref{tiling_c:1} 
and~\ref{tiling_c:2}. 
Thus, the formula $\atiling{k}{\cTT,\atile}$ is the one expressing all such properties. Once obtained, we are able to
prove~\Cref{lemma:tiling_correct_encoding}, and derive the following result.

\begin{theorem}\label{theorem:tower-completeness-SC}
  \satproblem{\modallogicSC}  is \tower-complete (\satproblem{\msokt} too).
\end{theorem}


==> sections/section-tiling-SC.tex <==
%!TEX root = ../main.tex
\subsection{Tiling a grid  $\interval{0}{\amapter(k,n)-1}  \times \interval{0}{\amapter(k,n)-1}$}\label{subsection:tiling-grid}
After the efforts needed in order to define the formula $\complete{j}$,
we are ready to  prove the \tower-hardness of
$\satproblem{\modallogicSC}$ with a uniform reduction from $\tiling_k$, for every $k \geq 2$.

Let $k \geq 2$ and let $\pair{\cTT}{\atile}$ be an instance of
$\tiling_k$, where $\cTT = \triple{\cT}{\cH}{\cV}$ and $\atile \in \cT$.
In the following, we define a formula $\atiling{k}{\cTT,\atile}$ such that the following lemma holds.

\begin{lemma}\label{lemma:tiling_correct_encoding}
$\pair{\cTT}{\atile}$ as a solution for $\tiling_k$ if and only if
the formula $\atiling{k}{\cTT,\atile}$ is satisfiable.
\end{lemma}

Recall that a solution for $\pair{\cTT}{\atile}$ w.r.t. $\tiling_k$ is a map
$\tau: \interval{0}{\amapter(k,n)-1}\!\times\!\interval{0}{\amapter(k,n)-1}\!\to\!\cT$
satisfying~\ref{tiling_c:1} and~\ref{tiling_c:2}.
W.l.o.g.\ we assume $\cT$ to be a set of atomic propositions, disjoint from
%% the sets
$\{\avarprop_1,\dots,\avarprop_n,\treeval\} \cup \Aux$ used in the definition of $\complete{j}$.
Let us first describe how to represent a grid $\interval{0}{\amapter(k,n)-1}^2$ in a pointed forest
$\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$.
We use the same ideas needed in order to define $\complete{k}$, but with some minor modifications.
As previously stated, if $\amodel,\aworld \models \complete{k}$ then
given a $\avartree$-node $\aworld' \in \arelation(\aworld)$,
the number $\nb{\aworld'} \in \interval{0}{\amapter(k,n)-1}$ is encoded using the $\avartree$-children of $\aworld'$, where the numbers encoded by these children represent positions
in the binary encoding of $\nb{\aworld'}$.
Instead of being a single number, a position in the grid is a pair of numbers  $(h,v) \in \interval{0}{\amapter(k,n)-1}^2$.
Hence, in a model $\pair{\amodel}{\aworld}$ satisfying $\atiling{k}{\cTT,\atile}$
we require that $\aworld' \in \arelation(\aworld)$ encodes two numbers $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$, and say that $\aworld'$ encodes the position $(h,v)$ if and only if $\nbexp{\aworld'}{\cH} = h$ and $\nbexp{\aworld'}{\cV} = v$.
Since both numbers are from $\interval{0}{\amapter(k,n)-1}$, the same amount of $\avartree$-children as in $\complete{k}$ can be used in order to encode both $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$.
Thus, we rely on the formula $\complete{k-1}$  to force $\aworld'$ to have the correct amount of $\avartree$-children, by requiring it to hold in $\pair{\amodel}{\aworld'}$.
Similarly to what done previously for $\complete{j}$ ($j \geq 2$), we encode the numbers $\nbexp{\aworld'}{\cH}$ and $\nbexp{\aworld'}{\cV}$
by using the truth value, on the $\avartree$-children of $\aworld'$, of two new atomic propositions $\treeval_\cH$ and $\treeval_\cV$, respectively.
Then, we  use similar formulae to $\pZ{k}$, $\pU{k}$ and $\pC{k}$ in order to state that $\aworld$ witness exactly one child for each position in the grid. Once the grid is encoded, the tiling conditions can be enforced rather easily.

We need to introduce the formula $\agrid{k}{\cTT}$ that characterises the set of models encoding the grid  $\interval{0}{\amapter(k,n)-1}^2$.
A model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying
$\agrid{k}{\cTT}$ is such that:
\begin{description}[noitemsep,topsep=0.5pt]
  \item[\desclabel{(\apZ$_{\cTT,k}$)}{tiling_enc:apZ}] one $\avartree$-node in $\arelation(\aworld)$ encodes the position $\pair{0}{0}$, i.e. there is an $\avartree$-node $\tilde\aworld{\in}\,\arelation(\aworld)$ s.t.\
    $\nbexp{\tilde\aworld}{\cH} = \nbexp{\tilde\aworld}{\cV} = 0$;
  \item[\desclabel{(\apU$_{\cTT,k}$)}{tiling_enc:apU}] for every two distinct $\avartree$-nodes $\aworld_1,\aworld_2 \in \arelation(\aworld)$, $\nbexp{\aworld_1}{\cH} \neq \nbexp{\aworld_2}{\cH}$ or  $\nbexp{\aworld_1}{\cH} \neq \nbexp{\aworld_2}{\cH}$;
  \item[\desclabel{(\apC$_{\cTT,k}$)}{tiling_enc:apC}] for every $\avartree$-node $\aworld_1 \in \arelation(\aworld)$,
  \begin{itemize}
    \item if $\nbexp{\aworld_1}{\cH} < \amapter(j,n)-1$ then $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}+1$ and $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}$, for some $\avartree$-node $\aworld_2 \in \arelation(\aworld)$;
    \item if $\nbexp{\aworld_1}{\cV} < \amapter(j,n)-1$ then $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}+1$ and $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}$, for some $\avartree$-node $\aworld_2 \in \arelation(\aworld)$;
  \end{itemize}
  \item[\desclabel{(\ainit/\apS/\apA)}{tiling_enc:apS}] $\pair{\amodel}{\aworld}$ satisfies $\init{k}$,  $\pS{k}$ and $\pA$.
\end{description}
It is easy to see that, with these conditions, $\pair{\amodel}{\aworld}$ correctly encodes the grid.
The definition of $\agrid{k}{\cTT}$ follows rather closely the definition of $\complete{j}$, and encodes the above-mentioned properties.
% It is defined as
% %\[
% \begin{nscenter}
%   $
%     \pZT{k}{\cTT} \land \pUT{k}{\cTT} \land \pCTBB{k}{\cTT} \land \init{k} \land \pS{k} \land \pA
%   $
% \end{nscenter}
% %\]
% where each conjunct express the homonymous property above.
% These formulae follow closely they definition of formulae in the previous section
% (due to lack of space, we skip the full definition).
%
% RF: for long version
%
% In order to define the first three conjuncts of $\agrid{k}{\cTT}$  (hence completing its definition)
% we start by defining the formulae $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ and $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$, where $\heapdim \in \{\cH,\cV\}$. Similarly to $\equivalent{\aaux}{\aauxbis}{1}{k}$ and $\successor{\aaux}{\aauxbis}{k}$,
% Given a model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying $\fork{\aaux}{\aauxbis}{1}{k}$, and the two $\avartree$-nodes $\aworld_{\aaux},\aworld_{\aauxbis} \in \arelation(\aworld)$
% corresponding to the nominals $\aaux$ and $\aauxbis$, respectively,
% \begin{itemize}
% \item $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ states that $\nbexp{\aworld_{\aaux}}{\heapdim} = \nbexp{\aworld_{\aauxbis}}{\heapdim}$;
% \item $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ states that $\nbexp{\aworld_{\aauxbis}}{\heapdim} = \nbexp{\aworld_{\aaux}}{\heapdim}+1$.
% \end{itemize}
% To encode $\bequivalent{\aaux}{\aauxbis}{k}{\heapdim}$ we simply require that for every two $\avartree$-children $\aworld_{\avariable} \in \arelation(\aworld_{\aaux})$ and $\aworld_{\avariablebis} \in \arelation(\aworld_{\aauxbis})$, if
% $\nb{\aworld_{\avariable}} = \nb{\aworld_{\avariablebis}}$ then $\aworld_{\avariable}$ and $\aworld_{\avariablebis}$
% agree on the satisfaction of $\treeval_\heapdim$. In formula:
% \[
% \begin{aligned}
%   \bequivalent{\aaux}{\aauxbis}{k}{\heapdim}
%   \egdef
%   \lnot \big( \true \separate & (\fork{\avariable}{\avariablebis}{2}{k}
%   \land \atnom{\aaux}{1}{\HMDiamond{\avartree} \Diamond \avariable}
%   \land \atnom{\aauxbis}{1}{\HMDiamond{\avartree} \Diamond \avariablebis}
%   \\ & \land \equivalent{\avariable}{\avariablebis}{2}{k}
%   \land \lnot (\atnom{\avariable}{2}\treeval_\heapdim \iff \atnom{\avariablebis}{2}\treeval_\heapdim)
%   )\big).
% \end{aligned}
% \]
% The formula $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ can be defined by slightly modifying the formula $\successor{\aaux}{\aauxbis}{k}$. We start by defining the formulae $\bleftpred{\aaux}{\aauxbis}{k}{\heapdim}$, $\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}$ and $\brightpred{\aaux}{\aauxbis}{\heapdim}$
% with semantics similar to $\leftpred{\aaux}{\aauxbis}{1}{k}$, $\selectpred{\aaux}{\aauxbis}{1}{k}$
% and $\rightpred{\aaux}{\aauxbis}$, respectively, but where, for a given $\avartree$-node in $\arelation^2(\aworld)$,
% we are interested in the satisfaction of $\treeval_\heapdim$ instead of $\treeval$. For example, the formula $\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}$ is defined as
% \[
% \begin{aligned}
%   & \bselectpred{\aaux}{\aauxbis}{k}{\heapdim}\egdef
%   \true \separate \big( \fork{\avariable}{\avariablebis}{2}{k} \land
%   \atnom{\aaux}{1}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariable)\, \land\\
%   &\ \ \atnom{\aauxbis}{1}\HMDiamond{\avartree}(\Diamond \avarselect \land \Diamond \avariablebis) \land \equivalent{\avariable}{\avariablebis}{2}{k} \land \atnom{\avariable}{2}\lnot \treeval_\heapdim \land \atnom{\avariablebis}{2}\treeval_\heapdim
%   \big)
% \end{aligned}
% \]
% i.e. by replacing the two last conjuncts of $\selectpred{\aaux}{\aauxbis}{1}{k}$, $\atnom{\avariable}{2}\lnot \treeval $ and $\atnom{\avariablebis}{2}\treeval$ with $\atnom{\avariable}{2}\lnot \treeval_\heapdim$ and $\atnom{\avariablebis}{2}\treeval_\heapdim$, respectively.
% Similarly, $\bleftpred{\aaux}{\aauxbis}{k}{\heapdim}$ is defined from $\leftpred{\aaux}{\aauxbis}{1}{k}$ by replacing the last conjunct of this formula, i.e.\ $\lnot (\atnom{\avariable}{2}\treeval \iff \atnom{\avariablebis}{2}\treeval)$, by
% $\lnot (\atnom{\avariable}{2}\treeval_\heapdim \iff \atnom{\avariablebis}{2}\treeval_\heapdim)$.
% Lastly, $\brightpred{\aaux}{\aauxbis}{\heapdim}$ is defined from $\rightpred{\aaux}{\aauxbis}$ by replacing every occurrence of $\treeval$ by $\treeval_\heapdim$.
% The formula $\bsuccessor{\aaux}{\aauxbis}{k}{\heapdim}$ is then defined as follows:
% \[
% \begin{aligned}
% \bsuccessor{\aaux}{\aauxbis}{k}{\heapdim} & \egdef
% \true \separate
%   \big(
%      \twonoms{\aaux}{\aauxbis}{1} \land \HMBox{\avartree}\lsrpartition{k-1} \land\\
%     & \ \, \bleftpred{\aaux}{\aauxbis}{k}{\heapdim}\,{\land}\,\bselectpred{\aaux}{\aauxbis}{k}{\heapdim}\,{\land}\,
%       \brightpred{\aaux}{\aauxbis}{\heapdim}
%   \big).
% \end{aligned}
% % \]
% We are now ready to define the formulae $\pZT{k}{\cTT}$, $\pUT{k}{\cTT}$ and $\pCTBB{k}{\cTT}$, achieving the conditions \ref{tiling_enc:apZ}, \ref{tiling_enc:apU} and \ref{tiling_enc:apC}, respectively.
% All these formulae follows closely the definitions of $\pZ{k}$, $\pU{k}$ and $\pC{k}$ of the previous sections, hence we refer to these latter formulae for an informal description on how they works. The formula $\pZT{k}{\cTT}$ is simply defined as $\HMDiamond{\avartree}(\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV))$.
% The formula $\pUT{k}{\cTT}$ is defined from $\pZ{k}$ by simply replacing $\equivalent{\avariable}{\avariablebis}{1}{k}$
% with $\bequivalent{\aaux}{\aauxbis}{k}{\cH} \land \bequivalent{\aaux}{\aauxbis}{k}{\cV}$:
% \[
% \pUT{k}{\cTT} = \lnot \big(\true \separate (\fork{\avariable}{\avariablebis}{1}{k} \land \bequivalent{\avariable}{\avariablebis}{k}{\cH} \land\bequivalent{\avariable}{\avariablebis}{k}{\cV})\big)
% \]
% Lastly, $\pCTBB{k}{\cTT} \egdef \pCTB{k}{\cTT}{\cH} \land \pCTB{k}{\cTT}{\cV}$ where
% \[
% \begin{aligned}
% &\pCTB{k}{\cTT}{\cH} \egdef \lnot
%   \Big( \Box \false\!\separate\!
%     \Big(\HMBox{\avartree} (\completeplus{k{-}1}\,{\land}\,\Diamond \avariablebis)\,{\land}\,
%     \nominal{\avariable}{1} \\
%  &\ \land
%  \atnom{\avariable}{1} \lnot \one^{\cH}_{k} \land \lnot \big( \true \separate (\fork{\avariable}{\avariablebis}{1}{j} \land
%  \bsuccessor{\avariable}{\avariablebis}{k}{\cH}
%  \land \bequivalent{\avariable}{\avariablebis}{k}{\cV}
%  )\big)\Big)\Big)
% \end{aligned}
% \]
% and $\pCTB{k}{\cTT}{\cV}$ is defined form $\pCTB{k}{\cTT}{\cH}$ by replacing $\one^{\cH}_{k}$, $\bsuccessor{\avariable}{\avariablebis}{k}{\cH}$ and
% $\bequivalent{\avariable}{\avariablebis}{k}{\cV}$ with
% $\one^{\cV}_{k}$, $\bsuccessor{\avariable}{\avariablebis}{k}{\cV}$ and
% $\bequivalent{\avariable}{\avariablebis}{k}{\cH}$, respectively.
% Here, $\one^{\heapdim}_{k}$ ($\heapdim \in \{\cH,\cV\}$) is defined as $\HMBox{\avartree} \treeval_\heapdim$,
% and hence it is satisfied by the $\avartree$-nodes $\aworld' \in \arelation(\aworld)$ such that $\nbexp{\aworld'}{\heapdim} = \amapter(k,n)-1$.
% This concludes the definition of $\agrid{k}{\cTT}$. It is proved correct in the following lemma.

% \begin{lemma}
% $\amodel,\aworld \models \agrid{k}{\cTT}$ if and only if $\pair{\amodel}{\aworld}$ satisfies \ref{tiling_enc:apZ}, \ref{tiling_enc:apU},
% \ref{tiling_enc:apC} and \ref{tiling_enc:apS}.
% \end{lemma}

% We can now proceed to the encoding of the tiling conditions~\ref{tiling_c:1} and~\ref{tiling_c:2}.
Additionally, we need to encode the tiling conditions~\ref{tiling_c:1} and~\ref{tiling_c:2}.
Given a model $\pair{\amodel = \triple{\worlds}{\arelation}{\avaluation}}{\aworld}$ satisfying
$\agrid{k}{\cTT}$, the existence of a solution for $\pair{\cTT}{\atile}$, w.r.t.\ $\tiling_k$, can be expressed with the following conditions:
\begin{description}[noitemsep,topsep=0.5pt]
  \item[\desclabel{(\apone$_{\cTT}$)}{tiling_enc:one_tile}] every $\avarprop$-node in $\arelation(\aworld)$ satisfies exactly one tile in $\cT$;
  \item[\desclabel{(\apfirst$_{\cTT,\atile}$)}{tiling_enc:zero_c}] for $\tilde\aworld{\in}\,\arelation(\aworld)$, if $\nbexp{\tilde\aworld}{\cH} {=} \nbexp{\tilde\aworld}{\cV} {=} 0$ then $\tilde{\aworld} \in \avaluation(\atile)$;
  \item [\desclabel{(\aphor$_{\cTT}$)}{tiling_enc:hori}] for all $\aworld_1,\aworld_2 \in \arelation(\aworld)$,
    if $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}+1$ and $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}$ then there is $\pair{\atile_1}{\atile_2} \in \cH$ such that
    $\aworld_1 \in \avaluation(\atile_1)$ and $\aworld_2 \in \avaluation(\atile_2)$;
  \item [\desclabel{(\apvert$_{\cTT}$)}{tiling_enc:hori}] for all $\aworld_1,\aworld_2 \in \arelation(\aworld)$,
    if $\nbexp{\aworld_2}{\cV} = \nbexp{\aworld_1}{\cV}+1$ and $\nbexp{\aworld_2}{\cH} = \nbexp{\aworld_1}{\cH}$ then there is $\pair{\atile_1}{\atile_2} \in \cV$ such that
    $\aworld_1 \in \avaluation(\atile_1)$ and $\aworld_2 \in \avaluation(\atile_2)$.
\end{description}
Then, the formula $\atiling{k}{\cTT,\atile}$ is the one expressing such properties, and again this can done rather easily given the toolkit of formulae introduced up to now.
%  can be defined as
% \[
% \agrid{k}{\cTT} \land \pone{\cTT} \land \pfirst{k}{\cTT,\atile} \land \phor{k}{\cTT} \land \pvert{k}{\cTT}
% \]
% where the last four conjuncts express the homonymous property above.
% Again, given the toolkit of formulae introduced up to now, these four formulae are easy to define.

% $\pone{\cTT}$ is simply defined as
% $\HMBox{\avartree}\bigvee_{\atile_1 \in \cT} (\atile_1 \land \bigwedge_{\atile_2 \in \cT} \lnot \atile_2)$.
% The formula $\pfirst{k}{\cTT,\atile}$ can be defined as
% \[
% \pfirst{k}{\cTT,\atile} \egdef \HMBox{\avartree}\big(\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV) \implies \atile\big)
% \]
% where we use the fact that
% the $\avartree$-node $\aworld' \in \arelation(\aworld)$ encoding $\pair{0}{0}$ is the only one, among the $\avartree$-children of $\aworld$, satisfying $\HMBox{\avartree}(\lnot \treeval_\cH \land \lnot \treeval_\cV)$.
% For the formula $\phor{k}{\cTT}$, we essentially state that there cannot be two $\avartree$-nodes $\aworld_1,\aworld_2 \in \arelation(\aworld)$ such that $\aworld_2$ encodes the position $\pair{\nbexp{\aworld_1}{\cH}+1}{\nbexp{\aworld_1}{\cV}}$
% and $\aworld_1 \in \avaluation(\atile_1)$, $\aworld_2 \in \avaluation(\atile_2)$ does not hold for any $\pair{\atile_1}{\atile_2} \in \cH$. In formula:
% \[
% \begin{aligned}
% \phor{k}{\cTT} \egdef \lnot
% \big(
% \true
%   \separate
%   \big(&
%   \fork{\avariable}{\avariablebis}{1}{k} \land
%   \bsuccessor{\avariable}{\avariablebis}{k}{\cH}
%   \land \bequivalent{\avariable}{\avariablebis}{k}{\cV}
%   \\
%   & \land
%   \lnot \textstyle\bigvee_{{\pair{\atile_1}{\atile_2} \in \cH}} (\atnom{\avariable}{1} \atile_1 \land \atnom{\avariablebis}{1} \atile_2)
%   \big)
% \big).
% \end{aligned}
% \]
% Lastly, $\pvert{k}{\cTT}$ is defined as $\phor{k}{\cTT}$, but replacing $\cH$ by $\cV$ and vice-versa
% (in particular, in $\pvert{k}{\cTT}$ the last disjunction appearing in $\phor{k}{\cTT}$ becomes indexed by elements in $\cV$).
% This conclude

Once we obtained the definition of $\atiling{k}{\cTT,\atile}$, we are able to prove Lemma~\ref{lemma:tiling_correct_encoding}.
We then derive the following result.

\begin{theorem}\label{theorem:tower-completeness-SC}
  $\satproblem{\modallogicSC}$ is \tower-complete.
\end{theorem}

